Birds of a Feather? Magellan/IMACS Spectroscopy of the Ultra-Faint Satellites Grus II, Tucana IV, and Tucana V

We present Magellan/IMACS spectroscopy of three recently discovered ultra-faint Milky Way satellites, Grus II, Tucana IV, and Tucana V. We measure systemic velocities of V_hel = -110.0 +/- 0.5 km/s, V_hel = 15.9 +/- 1.8 km/s, and V_hel = -36.2 +/-2.5 km/s for the three objects, respectively. Their large relative velocity differences demonstrate that the satellites are unrelated despite their close physical proximity. We determine a velocity dispersion for Tuc IV of sigma = 4.3^+1.7_-1.0 km/s, but we cannot resolve the velocity dispersions of the other two systems. For Gru II we place an upper limit (90% confidence) on the dispersion of sigma < 1.9 km/s, and for Tuc V we do not obtain any useful limits. All three satellites have metallicities below [Fe/H] = -2.1, but none has a detectable metallicity spread. We determine proper motions for each satellite based on Gaia astrometry and compute their orbits around the Milky Way. Gru II is on a tightly bound orbit with a pericenter of 25 kpc and orbital eccentricity of 0.45. Tuc V likely has an apocenter beyond 100 kpc, and could be approaching the Milky Way for the first time. The current orbit of Tuc IV is similar to that of Gru II, with a pericenter of 25 kpc and an eccentricity of 0.36. However, a backward integration of the position of Tuc IV demonstrates that it collided with the Large Magellanic Cloud at an impact parameter of 4 kpc ~120 Myr ago, deflecting its trajectory and possibly altering its internal kinematics. Based on their sizes, masses, and metallicities, we classify Gru II and Tuc IV as likely dwarf galaxies, but the nature of Tuc V remains uncertain.

==> aat_spec_table.tex <==
\LongTables

\tabletypesize{\scriptsize}
\begin{deluxetable*}{c c c c c c c r}
\tablecaption{AAT Velocity Measurements for Gru~II and Tuc~IV.\label{tab:aat}}

\tablehead{ID & MJD & RA & DEC & $g$\tablenotemark{a} & $r$\tablenotemark{a} & S/N & \multicolumn{1}{c}{$v$} \\ 
 &  & (deg) & (deg) & (mag) & (mag) &  & \multicolumn{1}{c}{(\kms)} }
\startdata
DES\,J215828.76$-$463329.6  &  57596.1  &  329.61985  & $ -46.55823 $ &  17.73  &  17.03  &    6.8  &    \phs$4.8 \pm 3.5$  \\
DES\,J215831.30$-$462702.6  &  57596.1  &  329.63040  & $ -46.45072 $ &  17.22  &  16.43  &   17.8  &      $-11.4 \pm 2.2$  \\
DES\,J215851.85$-$464030.5  &  57596.1  &  329.71605  & $ -46.67514 $ &  17.90  &  17.23  &    7.3  &      $-62.9 \pm 3.3$  \\
DES\,J215857.30$-$460420.0  &  57596.1  &  329.73874  & $ -46.07222 $ &  17.06  &  16.13  &   29.0  &      $-12.5 \pm 0.8$  \\
DES\,J215903.05$-$465407.6  &  57596.1  &  329.76272  & $ -46.90211 $ &  17.06  &  16.23  &    8.6  &      $-37.0 \pm 3.0$  \\
DES\,J215909.17$-$463536.3  &  57596.1  &  329.78819  & $ -46.59340 $ &  17.78  &  17.11  &    9.0  &       $-7.6 \pm 3.1$  \\
DES\,J215915.51$-$461956.4  &  57596.1  &  329.81464  & $ -46.33234 $ &  17.10  &  16.28  &   26.5  &      $-17.4 \pm 2.6$  \\
DES\,J215917.67$-$465605.9  &  57596.1  &  329.82361  & $ -46.93498 $ &  17.31  &  16.56  &    9.8  &   \phs$41.2 \pm 3.9$  \\
DES\,J215923.64$-$460638.6  &  57596.1  &  329.84849  & $ -46.11072 $ &  17.19  &  16.38  &   26.4  &      $-16.1 \pm 1.5$  \\
DES\,J215924.02$-$461309.8  &  57596.1  &  329.85008  & $ -46.21940 $ &  17.57  &  16.77  &   11.4  &   \phs$54.2 \pm 1.9$  \\
DES\,J215926.24$-$460748.6  &  57596.1  &  329.85935  & $ -46.13018 $ &  16.98  &  16.04  &   36.2  &      $-69.9 \pm 4.5$  \\
DES\,J215927.45$-$461621.4  &  57596.1  &  329.86438  & $ -46.27260 $ &  16.64  &  15.73  &   41.9  &      $-46.7 \pm 4.2$  \\
DES\,J215938.14$-$461220.5  &  57596.1  &  329.90893  & $ -46.20569 $ &  16.59  &  15.63  &   29.1  &   \phs$28.4 \pm 1.2$  \\
DES\,J215947.11$-$460208.7  &  57596.1  &  329.94628  & $ -46.03574 $ &  17.44  &  16.68  &   22.6  &      $-80.6 \pm 1.9$  \\
DES\,J220002.23$-$460906.8  &  57596.1  &  330.00929  & $ -46.15190 $ &  17.46  &  16.67  &   21.5  &      $-61.8 \pm 2.0$  \\
DES\,J220008.54$-$470757.1  &  57596.1  &  330.03559  & $ -47.13254 $ &  17.83  &  17.08  &    7.3  &     $-110.1 \pm 3.6$  \\
DES\,J220016.41$-$460714.8  &  57596.1  &  330.06836  & $ -46.12077 $ &  17.51  &  16.69  &   19.3  &   \phs$36.3 \pm 1.6$  \\
DES\,J220018.86$-$460919.8  &  57596.1  &  330.07857  & $ -46.15550 $ &  17.46  &  16.74  &   19.8  &   \phs$87.4 \pm 3.1$  \\
DES\,J220019.03$-$463330.1  &  57596.1  &  330.07927  & $ -46.55836 $ &  17.71  &  17.02  &   13.5  &      $-43.1 \pm 2.4$  \\
DES\,J220020.91$-$460305.7  &  57596.1  &  330.08711  & $ -46.05158 $ &  16.94  &  16.07  &   30.4  &       $-0.7 \pm 0.8$  \\
DES\,J220032.78$-$461840.5  &  57596.1  &  330.13658  & $ -46.31125 $ &  17.39  &  16.66  &   15.8  &      $-17.5 \pm 1.8$  \\
DES\,J220042.64$-$463138.8  &  57596.1  &  330.17767  & $ -46.52745 $ &  17.33  &  16.58  &   16.7  &    \phs$0.6 \pm 1.3$  \\
DES\,J220047.80$-$454956.3  &  57596.1  &  330.19918  & $ -45.83231 $ &  17.87  &  17.21  &   11.1  &      $-15.2 \pm 1.8$  \\
DES\,J220052.30$-$455445.1  &  57596.1  &  330.21792  & $ -45.91252 $ &  16.67  &  15.79  &   28.0  &      $-85.2 \pm 1.2$  \\
DES\,J220055.14$-$461650.2  &  57596.1  &  330.22977  & $ -46.28060 $ &  18.69  &  18.06  &    6.1  &      $-14.5 \pm 3.9$  \\
DES\,J220101.52$-$464447.7  &  57596.1  &  330.25635  & $ -46.74659 $ &  17.10  &  16.22  &   24.6  &      $-71.3 \pm 1.9$  \\
DES\,J220119.02$-$463207.6  &  57596.1  &  330.32927  & $ -46.53545 $ &  17.93  &  17.19  &    9.9  &    \phs$4.8 \pm 2.8$  \\
DES\,J220125.42$-$454319.5  &  57596.1  &  330.35591  & $ -45.72209 $ &  16.94  &  16.03  &   25.4  &   \phs$42.9 \pm 1.2$  \\
DES\,J220125.61$-$460156.9  &  57596.1  &  330.35669  & $ -46.03246 $ &  16.64  &  15.72  &   36.3  &      $-39.7 \pm 0.7$  \\
DES\,J220135.63$-$460841.9  &  57596.1  &  330.39846  & $ -46.14497 $ &  16.67  &  15.71  &   31.2  &      $-28.0 \pm 2.2$  \\
DES\,J220142.43$-$455851.6  &  57596.1  &  330.42679  & $ -45.98101 $ &  18.61  &  18.01  &    6.9  &      $-86.0 \pm 3.6$  \\
DES\,J220146.41$-$465911.1  &  57596.1  &  330.44337  & $ -46.98642 $ &  17.38  &  16.58  &   14.3  &   \phs$14.3 \pm 1.7$  \\
DES\,J220153.49$-$464603.7  &  57596.1  &  330.47287  & $ -46.76771 $ &  18.72  &  18.10  &    6.5  &   \phs$43.5 \pm 3.6$  \\
DES\,J220158.36$-$460259.2  &  57596.1  &  330.49316  & $ -46.04977 $ &  17.22  &  16.44  &   20.5  &      $-35.6 \pm 1.4$  \\
DES\,J220205.01$-$453952.7  &  57596.1  &  330.52088  & $ -45.66464 $ &  17.30  &  16.44  &   20.2  &   \phs$16.4 \pm 1.8$  \\
DES\,J220208.23$-$472045.0  &  57596.1  &  330.53428  & $ -47.34582 $ &  17.24  &  16.47  &   13.4  &       $-4.4 \pm 2.1$  \\
DES\,J220210.73$-$462111.9  &  57596.1  &  330.54472  & $ -46.35329 $ &  18.68  &  18.03  &    7.4  &   \phs$56.7 \pm 4.1$  \\
DES\,J220217.06$-$460631.7  &  57596.1  &  330.57108  & $ -46.10880 $ &  17.53  &  16.75  &   20.6  &      $-35.3 \pm 4.3$  \\
DES\,J220224.90$-$462417.9  &  57596.1  &  330.60375  & $ -46.40498 $ &  17.78  &  17.00  &   13.9  &   \phs$29.4 \pm 2.3$  \\
DES\,J220229.12$-$461649.2  &  57596.1  &  330.62133  & $ -46.28032 $ &  16.72  &  15.86  &   34.8  &     $-120.6 \pm 1.7$  \\
DES\,J220233.41$-$462321.0  &  57596.1  &  330.63923  & $ -46.38916 $ &  18.50  &  17.90  &    7.1  &   \phs$38.8 \pm 2.2$  \\
DES\,J220236.37$-$460754.4  &  57596.1  &  330.65154  & $ -46.13177 $ &  17.31  &  16.53  &   21.0  &      $-68.7 \pm 3.3$  \\
DES\,J220239.70$-$463923.0  &  57596.1  &  330.66542  & $ -46.65638 $ &  17.20  &  16.43  &   12.5  &   \phs$21.0 \pm 4.0$  \\
DES\,J220243.75$-$465204.1  &  57596.1  &  330.68230  & $ -46.86780 $ &  17.83  &  17.12  &   11.2  &   \phs$10.8 \pm 2.2$  \\
DES\,J220250.75$-$463003.9  &  57596.1  &  330.71148  & $ -46.50108 $ &  17.82  &  17.11  &   13.0  &      $-57.4 \pm 2.1$  \\
DES\,J220252.85$-$460802.3  &  57596.1  &  330.72022  & $ -46.13396 $ &  18.41  &  17.78  &    9.1  &     $-103.8 \pm 2.8$  \\
DES\,J220253.18$-$461413.3  &  57596.1  &  330.72157  & $ -46.23702 $ &  18.30  &  17.67  &    7.7  &   \phs$41.1 \pm 2.9$  \\
DES\,J220307.96$-$464750.0  &  57596.1  &  330.78317  & $ -46.79721 $ &  18.28  &  17.61  &    6.2  &       $-7.2 \pm 4.6$  \\
DES\,J220309.13$-$472052.9  &  57596.1  &  330.78804  & $ -47.34803 $ &  17.32  &  16.53  &    6.1  &    \phs$3.1 \pm 4.5$  \\
DES\,J220311.09$-$462116.2  &  57596.1  &  330.79622  & $ -46.35451 $ &  16.57  &  15.67  &   37.9  &   \phs$17.2 \pm 1.0$  \\
DES\,J220311.26$-$471731.0  &  57596.1  &  330.79692  & $ -47.29195 $ &  16.57  &  15.62  &   19.8  &    \phs$7.2 \pm 2.2$  \\
DES\,J220311.97$-$465758.5  &  57596.1  &  330.79989  & $ -46.96624 $ &  17.76  &  17.02  &   13.4  &   \phs$75.6 \pm 2.3$  \\
DES\,J220313.41$-$463119.9  &  57596.1  &  330.80587  & $ -46.52219 $ &  18.61  &  17.96  &    6.6  &   \phs$33.9 \pm 3.6$  \\
DES\,J220316.34$-$465227.0  &  57596.1  &  330.81808  & $ -46.87416 $ &  18.36  &  17.68  &    7.3  &       $-1.9 \pm 2.5$  \\
DES\,J220320.46$-$461300.9  &  57596.1  &  330.83524  & $ -46.21692 $ &  18.39  &  17.73  &    9.2  &      $-26.6 \pm 2.7$  \\
DES\,J220321.47$-$455729.7  &  57596.1  &  330.83945  & $ -45.95824 $ &  17.32  &  16.44  &   21.1  &   \phs$33.5 \pm 1.9$  \\
DES\,J220323.47$-$462156.4  &  57596.1  &  330.84780  & $ -46.36568 $ &  18.15  &  17.44  &   13.3  &   \phs$38.6 \pm 1.6$  \\
DES\,J220324.36$-$461213.5  &  57596.1  &  330.85150  & $ -46.20376 $ &  18.02  &  17.28  &   12.6  &    \phs$5.6 \pm 2.1$  \\
DES\,J220326.51$-$471030.0  &  57596.1  &  330.86045  & $ -47.17500 $ &  16.95  &  16.06  &   16.9  &      $-21.6 \pm 2.6$  \\
DES\,J220327.20$-$472137.4  &  57596.1  &  330.86332  & $ -47.36039 $ &  16.98  &  16.15  &    6.2  &      $-15.2 \pm 4.0$  \\
DES\,J220336.21$-$464527.4  &  57596.1  &  330.90087  & $ -46.75760 $ &  17.22  &  16.31  &   24.1  &      $-5.3 \pm 24.2$  \\
DES\,J220339.31$-$461422.6  &  57596.1  &  330.91379  & $ -46.23962 $ &  17.32  &  16.51  &   25.4  &    \phs$2.1 \pm 0.9$  \\
DES\,J220341.25$-$454826.0  &  57596.1  &  330.92186  & $ -45.80723 $ &  18.37  &  17.68  &   10.2  &      $-34.3 \pm 4.2$  \\
DES\,J220342.70$-$461843.3  &  57596.1  &  330.92791  & $ -46.31202 $ &  17.25  &  16.35  &   28.3  &      $-28.9 \pm 0.9$  \\
DES\,J220343.58$-$455908.6  &  57596.1  &  330.93157  & $ -45.98572 $ &  16.74  &  15.88  &   26.8  &    \phs$1.6 \pm 1.1$  \\
DES\,J220346.12$-$453249.1  &  57596.1  &  330.94216  & $ -45.54696 $ &  17.63  &  16.91  &   15.7  &      $-39.4 \pm 1.4$  \\
DES\,J220349.73$-$463314.6  &  57596.1  &  330.95722  & $ -46.55405 $ &  16.70  &  15.78  &   31.4  &       $-6.0 \pm 1.0$  \\
DES\,J220352.05$-$461213.5  &  57596.1  &  330.96689  & $ -46.20374 $ &  18.59  &  18.01  &    6.4  &      $-78.1 \pm 3.1$  \\
DES\,J220352.60$-$453309.7  &  57596.1  &  330.96916  & $ -45.55268 $ &  17.67  &  17.00  &   16.8  &       $-3.1 \pm 2.9$  \\
DES\,J220357.67$-$453907.0  &  57596.1  &  330.99029  & $ -45.65194 $ &  18.40  &  17.75  &   10.8  &  \phs$111.8 \pm 4.3$  \\
DES\,J220403.03$-$464422.9  &  57596.1  &  331.01262  & $ -46.73969 $ &  18.37  &  17.71  &    7.8  &      $-22.0 \pm 7.6$  \\
DES\,J220403.26$-$462403.3  &  57596.1  &  331.01359  & $ -46.40092 $ &  18.59  &  17.94  &    8.1  &       $-3.4 \pm 9.4$  \\
DES\,J220403.37$-$464925.4  &  57596.1  &  331.01405  & $ -46.82372 $ &  17.03  &  16.21  &   24.2  &    \phs$3.3 \pm 1.3$  \\
DES\,J220405.91$-$462231.3  &  57596.1  &  331.02461  & $ -46.37535 $ &  18.19  &  17.55  &   10.6  &   \phs$49.6 \pm 2.8$  \\
DES\,J220409.58$-$470421.1  &  57596.1  &  331.03993  & $ -47.07253 $ &  17.28  &  16.47  &   15.3  &   \phs$83.0 \pm 3.6$  \\
DES\,J220409.98$-$462102.2  &  57596.1  &  331.04158  & $ -46.35061 $ &  18.19  &  17.49  &   12.5  &     $-106.7 \pm 3.7$  \\
DES\,J220410.77$-$463202.5  &  57596.1  &  331.04486  & $ -46.53403 $ &  17.37  &  16.54  &   19.7  &   \phs$59.3 \pm 1.5$  \\
DES\,J220412.68$-$463502.8  &  57596.1  &  331.05283  & $ -46.58412 $ &  17.54  &  16.77  &   18.6  &   \phs$75.2 \pm 1.8$  \\
DES\,J220413.94$-$465754.5  &  57596.1  &  331.05807  & $ -46.96513 $ &  16.98  &  16.14  &   28.4  &       $-3.6 \pm 1.5$  \\
DES\,J220414.67$-$455356.9  &  57596.1  &  331.06112  & $ -45.89913 $ &  16.92  &  16.01  &   36.3  &   \phs$70.0 \pm 1.9$  \\
DES\,J220415.84$-$462454.9  &  57596.1  &  331.06599  & $ -46.41524 $ &  18.33  &  17.71  &    8.9  &       $-3.8 \pm 5.8$  \\
DES\,J220418.80$-$471226.4  &  57596.1  &  331.07833  & $ -47.20732 $ &  17.35  &  16.50  &   18.2  &    \phs$8.7 \pm 2.1$  \\
DES\,J220419.17$-$462831.5  &  57596.1  &  331.07987  & $ -46.47541 $ &  18.49  &  17.91  &    8.2  &      $-55.3 \pm 2.8$  \\
DES\,J220423.91$-$463702.5  &  57596.1  &  331.09961  & $ -46.61735 $ &  17.55  &  16.76  &   16.7  &     $-107.3 \pm 2.1$  \\
DES\,J220428.60$-$461736.1  &  57596.1  &  331.11916  & $ -46.29335 $ &  17.72  &  17.01  &   13.4  &     $-100.3 \pm 3.6$  \\
DES\,J220429.95$-$464045.0  &  57596.1  &  331.12478  & $ -46.67918 $ &  17.96  &  17.27  &   10.4  &      $-70.1 \pm 4.3$  \\
DES\,J220430.12$-$454619.2  &  57596.1  &  331.12551  & $ -45.77199 $ &  18.40  &  17.77  &   11.0  &   \phs$50.4 \pm 3.6$  \\
DES\,J220432.64$-$464456.7  &  57596.1  &  331.13601  & $ -46.74907 $ &  17.84  &  17.10  &   12.8  &   \phs$13.4 \pm 2.5$  \\
DES\,J220433.73$-$470950.8  &  57596.1  &  331.14052  & $ -47.16410 $ &  17.56  &  16.84  &    6.9  &   \phs$43.0 \pm 2.4$  \\
DES\,J220441.99$-$461605.5  &  57596.1  &  331.17498  & $ -46.26818 $ &  17.04  &  16.11  &   30.7  &       $-3.5 \pm 1.3$  \\
DES\,J220446.26$-$454240.7  &  57596.1  &  331.19273  & $ -45.71131 $ &  17.79  &  17.11  &   13.8  &      $-13.9 \pm 1.8$  \\
DES\,J220449.32$-$463042.6  &  57596.1  &  331.20551  & $ -46.51184 $ &  18.32  &  17.61  &    8.4  &    \phs$5.5 \pm 9.5$  \\
DES\,J220451.92$-$461845.9  &  57596.1  &  331.21633  & $ -46.31274 $ &  17.85  &  17.13  &   14.1  &      $-39.5 \pm 3.1$  \\
DES\,J220454.26$-$463443.4  &  57596.1  &  331.22610  & $ -46.57873 $ &  18.13  &  17.46  &    6.0  &      $-69.7 \pm 3.4$  \\
DES\,J220501.56$-$453734.7  &  57596.1  &  331.25651  & $ -45.62631 $ &  17.71  &  16.97  &   16.2  &      $-41.3 \pm 1.4$  \\
DES\,J220502.86$-$460947.5  &  57596.1  &  331.26192  & $ -46.16319 $ &  18.76  &  18.19  &    6.5  &      $-23.3 \pm 4.2$  \\
DES\,J220503.12$-$463234.7  &  57596.1  &  331.26300  & $ -46.54299 $ &  18.39  &  17.71  &    9.0  &      $-27.4 \pm 2.3$  \\
DES\,J220507.31$-$465032.7  &  57596.1  &  331.28046  & $ -46.84243 $ &  18.56  &  17.91  &    7.0  &    \phs$5.6 \pm 4.4$  \\
DES\,J220514.98$-$455626.9  &  57596.1  &  331.31240  & $ -45.94081 $ &  17.88  &  17.22  &   12.7  &      $-24.9 \pm 2.7$  \\
DES\,J220515.64$-$463736.5  &  57596.1  &  331.31515  & $ -46.62680 $ &  17.34  &  16.61  &   16.2  &   \phs$83.0 \pm 2.3$  \\
DES\,J220517.61$-$460933.5  &  57596.1  &  331.32338  & $ -46.15932 $ &  17.65  &  16.88  &   17.4  &   \phs$28.7 \pm 1.3$  \\
DES\,J220521.89$-$470230.5  &  57596.1  &  331.34119  & $ -47.04182 $ &  17.44  &  16.63  &   18.2  &      $-25.3 \pm 4.1$  \\
DES\,J220531.93$-$465858.9  &  57596.1  &  331.38304  & $ -46.98304 $ &  18.09  &  17.40  &   10.1  &   \phs$28.4 \pm 2.4$  \\
DES\,J220538.59$-$462007.1  &  57596.1  &  331.41081  & $ -46.33532 $ &  17.72  &  17.05  &   12.6  &      $-52.0 \pm 2.5$  \\
DES\,J220555.60$-$465905.8  &  57596.1  &  331.48165  & $ -46.98494 $ &  17.08  &  16.14  &   26.2  &   \phs$30.8 \pm 1.6$  \\
DES\,J220603.91$-$464009.9  &  57596.1  &  331.51629  & $ -46.66943 $ &  16.59  &  15.65  &   37.1  &      $-68.8 \pm 1.8$  \\
DES\,J220606.30$-$462600.7  &  57596.1  &  331.52624  & $ -46.43352 $ &  18.24  &  17.53  &   10.8  &   \phs$22.3 \pm 2.4$  \\
DES\,J220620.34$-$453423.1  &  57596.1  &  331.58475  & $ -45.57308 $ &  16.95  &  16.08  &   19.9  &     $-163.9 \pm 1.2$  \\
DES\,J220634.83$-$463611.2  &  57596.1  &  331.64514  & $ -46.60311 $ &  17.53  &  16.84  &   20.6  &      $-31.4 \pm 3.2$  \\
DES\,J220637.04$-$460935.6  &  57596.1  &  331.65433  & $ -46.15989 $ &  18.40  &  17.75  &    7.9  &      $-45.3 \pm 3.7$  \\
DES\,J220638.02$-$465827.8  &  57596.1  &  331.65841  & $ -46.97439 $ &  18.47  &  17.84  &    6.0  &      $-41.8 \pm 3.7$  \\
DES\,J220639.06$-$460644.3  &  57596.1  &  331.66275  & $ -46.11229 $ &  17.42  &  16.71  &   17.5  &   \phs$41.2 \pm 2.7$  \\
DES\,J220643.83$-$454652.6  &  57596.1  &  331.68264  & $ -45.78129 $ &  17.12  &  16.22  &   20.4  &    \phs$3.6 \pm 2.6$  \\
DES\,J220645.99$-$461925.9  &  57596.1  &  331.69162  & $ -46.32385 $ &  16.84  &  15.97  &   34.4  &   \phs$12.3 \pm 6.2$  \\
DES\,J220650.45$-$454307.2  &  57596.1  &  331.71019  & $ -45.71866 $ &  16.58  &  15.68  &   28.0  &      $-43.6 \pm 1.8$  \\
DES\,J220657.46$-$470940.7  &  57596.1  &  331.73943  & $ -47.16131 $ &  17.78  &  17.11  &    8.0  &   \phs$14.6 \pm 2.7$  \\
DES\,J220701.26$-$465942.3  &  57596.1  &  331.75527  & $ -46.99508 $ &  16.91  &  16.03  &   21.4  &   \phs$50.9 \pm 1.0$  \\
DES\,J220703.79$-$463456.0  &  57596.1  &  331.76580  & $ -46.58223 $ &  17.92  &  17.19  &   10.3  &       $-0.6 \pm 1.8$  \\
DES\,J220706.40$-$462254.3  &  57596.1  &  331.77666  & $ -46.38175 $ &  18.84  &  18.24  &    6.6  &     $-144.6 \pm 3.6$  \\
DES\,J220714.47$-$461357.5  &  57596.1  &  331.81030  & $ -46.23263 $ &  18.24  &  17.58  &    9.7  &    \phs$4.0 \pm 3.3$  \\
DES\,J220733.19$-$460747.0  &  57596.1  &  331.88827  & $ -46.12972 $ &  17.69  &  17.00  &   14.4  &      $-13.6 \pm 1.8$  \\
DES\,J220736.17$-$460448.2  &  57596.1  &  331.90072  & $ -46.08007 $ &  17.59  &  16.83  &   17.7  &     $-156.2 \pm 2.0$  \\
DES\,J220740.00$-$463100.9  &  57596.1  &  331.91665  & $ -46.51692 $ &  16.80  &  15.90  &   33.5  &   \phs$52.2 \pm 1.2$  \\
DES\,J220759.01$-$463111.2  &  57596.1  &  331.99587  & $ -46.51979 $ &  18.58  &  17.94  &    6.0  &      $-40.9 \pm 4.7$  \\
DES\,J220804.87$-$462705.5  &  57596.1  &  332.02029  & $ -46.45152 $ &  17.03  &  16.22  &   16.3  &       $-2.5 \pm 1.3$  \\
DES\,J220805.76$-$463506.5  &  57596.1  &  332.02400  & $ -46.58515 $ &  16.60  &  15.68  &   40.1  &   \phs$44.5 \pm 0.7$  \\
DES\,J220822.55$-$461131.9  &  57596.1  &  332.09397  & $ -46.19219 $ &  17.81  &  17.12  &   11.4  &     $-126.0 \pm 2.4$  \\
DES\,J220845.37$-$463236.7  &  57596.1  &  332.18905  & $ -46.54352 $ &  16.95  &  16.10  &   22.0  &    \phs$9.6 \pm 1.2$  \\
DES\,J220904.59$-$463834.0  &  57596.1  &  332.26914  & $ -46.64277 $ &  17.55  &  16.81  &   12.6  &      $-48.4 \pm 2.0$  \\
DES\,J235504.91$-$604802.5  &  57596.6  &  358.77045  & $ -60.80069 $ &  16.43  &  15.53  &   23.6  &      $-10.4 \pm 0.8$  \\
DES\,J235514.57$-$605359.6  &  57596.6  &  358.81069  & $ -60.89989 $ &  16.56  &  15.67  &   21.9  &      $-17.5 \pm 1.4$  \\
DES\,J235538.24$-$603942.9  &  57596.6  &  358.90935  & $ -60.66191 $ &  16.97  &  16.18  &   12.6  &   \phs$19.7 \pm 1.7$  \\
DES\,J235626.91$-$603046.5  &  57596.6  &  359.11214  & $ -60.51291 $ &  17.57  &  16.90  &    7.1  &   \phs$23.0 \pm 2.5$  \\
DES\,J235628.70$-$602045.9  &  57596.6  &  359.11959  & $ -60.34608 $ &  17.03  &  16.25  &   12.2  &      $-35.7 \pm 2.8$  \\
DES\,J235642.94$-$605316.6  &  57596.6  &  359.17892  & $ -60.88796 $ &  16.27  &  15.29  &   22.8  &      $-10.4 \pm 1.0$  \\
DES\,J235647.57$-$612136.3  &  57596.6  &  359.19822  & $ -61.36007 $ &  16.97  &  16.13  &   17.5  &      $-38.2 \pm 1.0$  \\
DES\,J235714.80$-$612348.2  &  57596.6  &  359.31168  & $ -61.39671 $ &  16.74  &  15.83  &   22.7  &   \phs$21.5 \pm 3.4$  \\
DES\,J235801.89$-$604617.7  &  57596.6  &  359.50789  & $ -60.77159 $ &  16.72  &  15.79  &   20.8  &      $-20.6 \pm 1.3$  \\
DES\,J235803.60$-$601021.6  &  57596.6  &  359.51502  & $ -60.17267 $ &  16.73  &  15.82  &   15.8  &      $-33.8 \pm 1.3$  \\
DES\,J235834.08$-$611746.6  &  57596.6  &  359.64201  & $ -61.29627 $ &  16.75  &  15.88  &   23.3  &      $-31.3 \pm 1.0$  \\
DES\,J235838.45$-$604412.2  &  57596.6  &  359.66022  & $ -60.73671 $ &  17.69  &  17.00  &    8.5  &   \phs$57.4 \pm 3.3$  \\
DES\,J235853.59$-$600600.2  &  57596.6  &  359.72329  & $ -60.10006 $ &  16.84  &  16.03  &   15.5  &   \phs$16.3 \pm 1.1$  \\
DES\,J235918.25$-$611722.6  &  57596.6  &  359.82603  & $ -61.28961 $ &  17.23  &  16.48  &   15.9  &    \phs$9.0 \pm 1.4$  \\
DES\,J235959.66$-$603205.9  &  57596.6  &  359.99857  & $ -60.53498 $ &  17.49  &  16.80  &   12.5  &      $-50.7 \pm 2.0$  \\
DES\,J000000.18$-$605741.3  &  57596.6  &    0.00074  & $ -60.96148 $ &  17.72  &  17.02  &   10.4  &   \phs$36.5 \pm 2.4$  \\
DES\,J000005.16$-$613245.5  &  57596.6  &    0.02149  & $ -61.54598 $ &  17.07  &  16.25  &   11.3  &   \phs$16.0 \pm 1.6$  \\
DES\,J000014.10$-$602051.6  &  57596.6  &    0.05875  & $ -60.34767 $ &  16.83  &  15.96  &   18.8  &   \phs$25.1 \pm 0.7$  \\
DES\,J000015.17$-$603540.0  &  57596.6  &    0.06323  & $ -60.59444 $ &  16.21  &  15.25  &   32.5  &   \phs$17.1 \pm 0.7$  \\
DES\,J000024.30$-$605819.6  &  57596.6  &    0.10124  & $ -60.97211 $ &  17.69  &  16.99  &   11.3  &   \phs$25.8 \pm 1.7$  \\
DES\,J000030.48$-$602634.4  &  57596.6  &    0.12701  & $ -60.44289 $ &  16.96  &  16.19  &   15.8  &   \phs$13.5 \pm 1.3$  \\
DES\,J000050.56$-$614128.0  &  57596.6  &    0.21067  & $ -61.69110 $ &  17.43  &  16.66  &   10.7  &      $-27.5 \pm 2.1$  \\
DES\,J000052.40$-$605930.3  &  57596.6  &    0.21834  & $ -60.99174 $ &  17.06  &  16.21  &   18.9  &    \phs$8.6 \pm 1.6$  \\
DES\,J000110.36$-$604246.0  &  57596.6  &    0.29315  & $ -60.71278 $ &  18.20  &  17.54  &    7.0  &   \phs$99.4 \pm 4.9$  \\
DES\,J000120.17$-$600155.4  &  57596.6  &    0.33403  & $ -60.03205 $ &  17.57  &  16.90  &    9.1  &      $-56.2 \pm 2.4$  \\
DES\,J000120.28$-$603918.3  &  57596.6  &    0.33449  & $ -60.65508 $ &  17.18  &  16.42  &   17.2  &   \phs$12.7 \pm 1.7$  \\
DES\,J000123.25$-$603433.7  &  57596.6  &    0.34686  & $ -60.57603 $ &  17.64  &  16.96  &   10.8  &        $0.0 \pm 2.2$  \\
DES\,J000129.34$-$603542.5  &  57596.6  &    0.37224  & $ -60.59513 $ &  18.28  &  17.62  &    7.2  &       $-1.9 \pm 4.3$  \\
DES\,J000129.95$-$610230.1  &  57596.6  &    0.37479  & $ -61.04168 $ &  17.93  &  17.26  &    9.4  &  \phs$213.6 \pm 4.3$  \\
DES\,J000130.40$-$610737.8  &  57596.6  &    0.37666  & $ -61.12717 $ &  17.38  &  16.58  &   14.1  &      $-39.2 \pm 2.0$  \\
DES\,J000140.26$-$613560.0  &  57596.6  &    0.41774  & $ -61.59999 $ &  17.34  &  16.60  &   12.0  &   \phs$55.0 \pm 2.4$  \\
DES\,J000149.99$-$604346.9  &  57596.6  &    0.45828  & $ -60.72970 $ &  18.35  &  17.77  &    6.2  &   \phs$52.4 \pm 4.4$  \\
DES\,J000159.69$-$610715.8  &  57596.6  &    0.49869  & $ -61.12106 $ &  16.38  &  15.48  &   27.8  &   \phs$11.3 \pm 1.8$  \\
DES\,J000209.74$-$605907.1  &  57596.6  &    0.54059  & $ -60.98530 $ &  17.91  &  17.25  &   12.3  &  \phs$257.3 \pm 6.4$  \\
DES\,J000213.83$-$601931.9  &  57596.6  &    0.55764  & $ -60.32552 $ &  17.50  &  16.73  &   12.3  &   \phs$70.1 \pm 2.2$  \\
DES\,J000219.66$-$614520.9  &  57596.6  &    0.58192  & $ -61.75580 $ &  16.84  &  16.01  &   19.4  &       $-6.5 \pm 1.6$  \\
DES\,J000224.49$-$613428.6  &  57596.6  &    0.60205  & $ -61.57460 $ &  19.25  &  18.70  &    6.2  &   \phs$18.9 \pm 3.7$  \\
DES\,J000228.66$-$611002.5  &  57596.6  &    0.61943  & $ -61.16736 $ &  17.88  &  17.20  &    9.2  &   \phs$50.5 \pm 4.7$  \\
DES\,J000231.47$-$602107.5  &  57596.6  &    0.63114  & $ -60.35209 $ &  16.74  &  15.88  &   16.9  &      $-18.2 \pm 1.3$  \\
DES\,J000238.21$-$605419.3  &  57596.6  &    0.65921  & $ -60.90537 $ &  17.06  &  16.21  &   17.2  &   \phs$37.5 \pm 1.3$  \\
DES\,J000239.40$-$614552.4  &  57596.6  &    0.66415  & $ -61.76455 $ &  18.37  &  17.73  &    6.4  &   \phs$27.1 \pm 2.9$  \\
DES\,J000246.06$-$611308.3  &  57596.6  &    0.69190  & $ -61.21896 $ &  18.18  &  17.54  &    6.1  &  \phs$159.1 \pm 3.1$  \\
DES\,J000251.72$-$602640.8  &  57596.6  &    0.71551  & $ -60.44466 $ &  17.46  &  16.69  &    8.6  &   \phs$23.8 \pm 2.3$  \\
DES\,J000310.05$-$595439.4  &  57596.6  &    0.79189  & $ -59.91094 $ &  17.58  &  16.86  &    7.9  &      $-13.8 \pm 2.6$  \\
DES\,J000313.09$-$613905.6  &  57596.6  &    0.80456  & $ -61.65155 $ &  16.58  &  15.72  &   21.9  &    \phs$7.4 \pm 2.0$  \\
DES\,J000340.21$-$605420.5  &  57596.6  &    0.91752  & $ -60.90571 $ &  17.11  &  16.31  &   16.4  &      $-38.9 \pm 1.9$  \\
DES\,J000344.20$-$610112.0  &  57596.6  &    0.93415  & $ -61.01999 $ &  17.48  &  16.74  &   10.8  &       $-9.3 \pm 2.4$  \\
DES\,J000359.68$-$612742.6  &  57596.6  &    0.99867  & $ -61.46183 $ &  16.89  &  16.03  &   14.5  &      $-47.2 \pm 1.7$  \\
DES\,J000410.01$-$603453.8  &  57596.6  &    1.04173  & $ -60.58161 $ &  17.49  &  16.71  &   10.7  &  \phs$114.1 \pm 5.1$  \\
DES\,J000410.51$-$601703.6  &  57596.6  &    1.04380  & $ -60.28433 $ &  17.53  &  16.81  &    8.5  &  \phs$117.3 \pm 3.5$  \\
DES\,J000424.72$-$612904.9  &  57596.6  &    1.10300  & $ -61.48469 $ &  17.37  &  16.64  &   13.9  &    \phs$3.3 \pm 1.3$  \\
DES\,J000430.00$-$605643.5  &  57596.6  &    1.12499  & $ -60.94543 $ &  17.37  &  16.59  &   13.2  &       $-0.9 \pm 2.0$  \\
DES\,J000436.92$-$602713.5  &  57596.6  &    1.15384  & $ -60.45375 $ &  17.02  &  16.19  &   15.1  &       $-7.7 \pm 1.3$  \\
DES\,J000444.14$-$605431.7  &  57596.6  &    1.18391  & $ -60.90879 $ &  16.66  &  15.72  &   21.6  &   \phs$46.2 \pm 3.0$  \\
DES\,J000446.48$-$603132.5  &  57596.6  &    1.19367  & $ -60.52571 $ &  16.99  &  16.22  &   13.2  &   \phs$42.4 \pm 1.9$  \\
DES\,J000450.55$-$600419.7  &  57596.6  &    1.21064  & $ -60.07214 $ &  17.05  &  16.29  &   13.6  &   \phs$21.5 \pm 1.5$  \\
DES\,J000502.19$-$614302.7  &  57596.6  &    1.25913  & $ -61.71742 $ &  16.97  &  16.19  &   16.8  &       $-0.4 \pm 2.3$  \\
DES\,J000517.00$-$601345.1  &  57596.6  &    1.32084  & $ -60.22920 $ &  17.72  &  16.98  &   10.3  &   \phs$90.5 \pm 1.9$  \\
DES\,J000531.19$-$595439.0  &  57596.6  &    1.37996  & $ -59.91082 $ &  17.02  &  16.23  &    8.3  &   \phs$29.5 \pm 3.6$  \\
DES\,J000540.08$-$610507.4  &  57596.6  &    1.41702  & $ -61.08540 $ &  17.22  &  16.41  &   13.8  &    \phs$8.7 \pm 1.8$  \\
DES\,J000603.68$-$611712.8  &  57596.6  &    1.51533  & $ -61.28688 $ &  16.96  &  16.15  &   18.4  &       $-8.1 \pm 1.0$  \\
DES\,J000605.88$-$600648.4  &  57596.6  &    1.52450  & $ -60.11344 $ &  17.30  &  16.53  &   11.4  &   \phs$41.5 \pm 3.1$  \\
DES\,J000611.25$-$614330.7  &  57596.6  &    1.54687  & $ -61.72520 $ &  17.69  &  17.04  &    8.2  &    \phs$7.2 \pm 2.6$  \\
DES\,J000615.93$-$612914.6  &  57596.6  &    1.56639  & $ -61.48739 $ &  17.43  &  16.71  &   12.2  &   \phs$33.5 \pm 3.7$  \\
DES\,J000623.11$-$610210.0  &  57596.6  &    1.59627  & $ -61.03610 $ &  17.69  &  17.05  &    8.8  &       $-8.7 \pm 2.1$  \\
DES\,J000623.40$-$613407.2  &  57596.6  &    1.59750  & $ -61.56866 $ &  17.40  &  16.71  &   12.0  &   \phs$25.0 \pm 4.2$  \\
DES\,J000634.63$-$604752.5  &  57596.6  &    1.64428  & $ -60.79791 $ &  17.85  &  17.19  &    6.4  &   \phs$38.9 \pm 3.2$  \\
DES\,J000710.10$-$602255.7  &  57596.6  &    1.79207  & $ -60.38212 $ &  17.55  &  16.88  &    9.2  &   \phs$66.4 \pm 2.2$  \\
DES\,J000725.03$-$612202.7  &  57596.6  &    1.85427  & $ -61.36742 $ &  17.46  &  16.78  &   12.4  &      $-35.1 \pm 1.8$  \\
DES\,J000728.43$-$604313.3  &  57596.6  &    1.86844  & $ -60.72036 $ &  17.30  &  16.57  &   11.2  &  \phs$156.5 \pm 2.3$  \\
DES\,J000736.93$-$613121.8  &  57596.6  &    1.90388  & $ -61.52272 $ &  16.89  &  16.06  &   18.2  &   \phs$46.4 \pm 1.6$  \\
DES\,J000759.76$-$613310.5  &  57596.6  &    1.99900  & $ -61.55291 $ &  16.93  &  16.12  &    8.3  &    \phs$0.1 \pm 2.4$  \\
DES\,J000810.21$-$613336.4  &  57596.6  &    2.04256  & $ -61.56011 $ &  17.63  &  16.89  &    8.7  &      $-32.8 \pm 2.8$  \\
DES\,J000825.36$-$611536.4  &  57596.6  &    2.10565  & $ -61.26012 $ &  17.07  &  16.31  &   14.1  &      $-33.9 \pm 1.6$  \\
DES\,J000826.61$-$610816.0  &  57596.6  &    2.11087  & $ -61.13777 $ &  17.68  &  17.04  &   10.3  &  \phs$114.0 \pm 2.8$  \\
DES\,J000840.27$-$602524.6  &  57596.6  &    2.16779  & $ -60.42349 $ &  17.70  &  16.98  &    7.3  &      $-26.0 \pm 2.4$  \\
DES\,J000857.26$-$604725.6  &  57596.6  &    2.23857  & $ -60.79046 $ &  17.55  &  16.90  &    7.0  &  \phs$153.4 \pm 3.5$  \\
DES\,J000945.43$-$603059.2  &  57596.6  &    2.43927  & $ -60.51643 $ &  17.26  &  16.53  &   10.7  &   \phs$33.1 \pm 2.3$  \\
DES\,J001020.89$-$611707.0  &  57596.6  &    2.58704  & $ -61.28528 $ &  17.66  &  16.95  &    7.0  &   \phs$32.8 \pm 3.1$  \\
DES\,J001036.96$-$610752.7  &  57596.6  &    2.65400  & $ -61.13131 $ &  17.48  &  16.81  &    8.6  &      $-42.1 \pm 2.9$  \\
DES\,J001058.46$-$604542.2  &  57596.6  &    2.74357  & $ -60.76173 $ &  16.89  &  16.03  &   12.2  &    \phs$3.1 \pm 1.8$  \\
\enddata
\tablenotetext{a}{Quoted magnitudes represent the weighted-average dereddened PSF magnitude derived from the DES images using SExtractor \citep{drlica15}.}
\end{deluxetable*}


==> imacs_spec_table.tex <==
\LongTables

\tabletypesize{\scriptsize}
\begin{deluxetable*}{c c c c c c c r c c c}
\tablecaption{IMACS Velocity and Metallicity Measurements for Gru~II, Tuc~IV, and Tuc~V.\label{tab:imacs_spec_table}}

\tablehead{ID & RA & DEC & $g$\tablenotemark{a} & $r$\tablenotemark{a} & MJD & S/N & \multicolumn{1}{c}{$v$} & ${\rm EW}$ & ${\rm [Fe/H]}$ & Mem\tablenotemark{b} \\ 
 & (deg) & (deg) & (mag) & (mag) &  &  & \multicolumn{1}{c}{(\kms)} & (\AA) &  &  }
\startdata
DES\,J220255.41$-$462538.9  &  330.73088  & $ -46.42747 $ &  19.18  &  19.24  &  58363.6  &    5.9  &     $-104.4 \pm 3.3$  &         ...       &         ...        &  1 \\
DES\,J220304.94$-$462841.7  &  330.77059  & $ -46.47824 $ &  20.59  &  20.09  &  57282.6  &   11.8  &     $-142.7 \pm 4.1$  &  $5.98 \pm 0.61$  &         ...        &  0 \\
DES\,J220308.10$-$462259.2  &  330.78377  & $ -46.38312 $ &  20.15  &  19.25  &  58363.6  &    8.6  &  \phs$107.3 \pm 2.7$  &         ...       &         ...        &  0 \\
DES\,J220309.37$-$462634.2  &  330.78903  & $ -46.44283 $ &  18.44  &  17.57  &  58363.6  &   34.5  &   \phs$23.4 \pm 1.2$  &  $5.65 \pm 0.38$  &         ...        &  0 \\
DES\,J220309.47$-$463255.6  &  330.78944  & $ -46.54878 $ &  18.69  &  18.08  &  57282.6  &   45.7  &   \phs$40.4 \pm 1.2$  &  $5.75 \pm 0.36$  &         ...        &  0 \\
                            &  330.78944  & $ -46.54878 $ &  18.69  &  18.08  &  57634.4  &   18.4  &   \phs$41.8 \pm 1.5$  &  $5.76 \pm 0.49$  &         ...        &  0 \\
DES\,J220310.98$-$462848.8  &  330.79573  & $ -46.48023 $ &  18.78  &  18.43  &  58363.6  &   16.6  &   \phs$42.2 \pm 1.4$  &  $3.95 \pm 0.45$  &         ...        &  0 \\
DES\,J220311.39$-$462555.3  &  330.79746  & $ -46.43203 $ &  19.48  &  19.12  &  58363.6  &    8.3  &      $-18.3 \pm 1.7$  &  $2.56 \pm 0.55$  &         ...        &  0 \\
DES\,J220311.75$-$462652.7  &  330.79897  & $ -46.44796 $ &  21.15  &  20.64  &  57980.9  &    5.6  &   \phs$69.2 \pm 3.2$  &  $4.01 \pm 1.81$  &         ...        &  0 \\
DES\,J220312.90$-$463312.1  &  330.80374  & $ -46.55336 $ &  19.61  &  18.95  &  57282.6  &   26.1  &      $-13.9 \pm 1.4$  &  $5.75 \pm 0.41$  &         ...        &  0 \\
                            &  330.80374  & $ -46.55336 $ &  19.61  &  18.95  &  57634.4  &    8.4  &      $-16.0 \pm 2.9$  &         ...       &         ...        &  0 \\
DES\,J220313.41$-$462241.5  &  330.80588  & $ -46.37818 $ &  19.69  &  18.73  &  58363.6  &   14.9  &  \phs$122.4 \pm 1.4$  &  $5.61 \pm 0.57$  &         ...        &  0 \\
DES\,J220313.53$-$462621.9  &  330.80637  & $ -46.43942 $ &  20.03  &  19.64  &  58363.6  &    4.7  &   \phs$55.8 \pm 8.9$  &  $4.47 \pm 1.68$  &         ...        &  0 \\
DES\,J220314.13$-$463100.7  &  330.80889  & $ -46.51686 $ &  18.08  &  17.61  &  57282.6  &   61.8  &   \phs$28.9 \pm 1.2$  &  $5.18 \pm 0.33$  &         ...        &  0 \\
                            &  330.80889  & $ -46.51686 $ &  18.08  &  17.61  &  57634.4  &   26.6  &   \phs$27.9 \pm 1.2$  &  $4.87 \pm 0.39$  &         ...        &  0 \\
DES\,J220314.15$-$462843.3  &  330.80896  & $ -46.47870 $ &  21.01  &  20.65  &  57282.6  &    6.5  &      $-85.5 \pm 2.7$  &         ...       &         ...        &  0 \\
DES\,J220314.21$-$463009.5  &  330.80921  & $ -46.50264 $ &  20.82  &  20.64  &  57282.6  &    6.1  &  \phs$211.0 \pm 8.6$  &         ...       &         ...        &  0 \\
DES\,J220314.90$-$462411.5  &  330.81206  & $ -46.40319 $ &  20.57  &  19.60  &  58363.6  &    6.0  &   \phs$76.8 \pm 4.8$  &         ...       &         ...        &  0 \\
DES\,J220317.46$-$463422.5  &  330.82275  & $ -46.57291 $ &  20.11  &  20.02  &  57282.6  &    8.4  &    \phs$3.0 \pm 3.2$  &         ...       &         ...        &  0 \\
DES\,J220319.25$-$461704.8  &  330.83022  & $ -46.28466 $ &  20.53  &  19.98  &  57284.1  &    4.8  &    \phs$9.0 \pm 4.5$  &  $6.52 \pm 1.13$  &         ...        &  0 \\
                            &  330.83022  & $ -46.28466 $ &  20.53  &  19.98  &  57630.5  &    6.2  &   \phs$22.0 \pm 3.3$  &  $4.06 \pm 0.73$  &         ...        &  0 \\
DES\,J220320.45$-$462643.1  &  330.83523  & $ -46.44530 $ &  20.70  &  20.24  &  57282.6  &    8.7  &     $-107.7 \pm 2.2$  &  $1.93 \pm 0.51$  &  $-2.51 \pm 0.31$  &  1 \\
                            &  330.83523  & $ -46.44530 $ &  20.70  &  20.24  &  57980.9  &    8.8  &     $-112.2 \pm 1.8$  &         ...       &         ...        &  1 \\
DES\,J220320.50$-$461625.5  &  330.83540  & $ -46.27376 $ &  18.10  &  17.65  &  57284.1  &   28.4  &   \phs$83.2 \pm 1.4$  &         ...       &         ...        &  0 \\
                            &  330.83540  & $ -46.27376 $ &  18.10  &  17.65  &  57630.5  &   33.8  &   \phs$81.9 \pm 1.1$  &         ...       &         ...        &  0 \\
DES\,J220321.53$-$462959.8  &  330.83970  & $ -46.49995 $ &  21.09  &  20.20  &  57282.6  &   11.6  &       $-8.1 \pm 1.8$  &  $6.97 \pm 0.77$  &         ...        &  0 \\
                            &  330.83970  & $ -46.49995 $ &  21.09  &  20.20  &  57634.4  &    4.1  &    \phs$1.2 \pm 7.8$  &  $5.27 \pm 1.09$  &         ...        &  0 \\
DES\,J220321.61$-$462415.1  &  330.84004  & $ -46.40419 $ &  18.25  &  18.00  &  58363.6  &   19.8  &  \phs$266.3 \pm 1.4$  &  $2.46 \pm 0.44$  &         ...        &  0 \\
DES\,J220321.76$-$462903.4  &  330.84065  & $ -46.48428 $ &  18.95  &  18.65  &  57980.9  &   29.4  &   \phs$75.0 \pm 1.1$  &  $1.86 \pm 0.36$  &         ...        &  0 \\
                            &  330.84065  & $ -46.48428 $ &  18.95  &  18.65  &  58363.6  &   13.6  &   \phs$73.1 \pm 1.7$  &  $1.67 \pm 0.52$  &         ...        &  0 \\
DES\,J220323.47$-$462156.4  &  330.84780  & $ -46.36568 $ &  18.15  &  17.44  &  58363.6  &   30.4  &   \phs$40.9 \pm 1.1$  &  $6.50 \pm 0.40$  &         ...        &  0 \\
DES\,J220325.79$-$461617.0  &  330.85748  & $ -46.27139 $ &  20.69  &  20.22  &  57630.5  &    4.4  &      $-50.8 \pm 5.5$  &         ...       &         ...        &  0 \\
DES\,J220327.16$-$462556.8  &  330.86315  & $ -46.43243 $ &  19.47  &  19.26  &  57282.6  &   16.7  &      $-96.5 \pm 1.8$  &  $2.16 \pm 0.40$  &         ...        &  0 \\
                            &  330.86315  & $ -46.43243 $ &  19.47  &  19.26  &  57634.4  &    7.5  &      $-98.7 \pm 2.6$  &         ...       &         ...        &  0 \\
DES\,J220327.63$-$461331.2  &  330.86514  & $ -46.22534 $ &  20.95  &  20.49  &  57630.5  &    4.2  &   \phs$16.9 \pm 2.7$  &  $4.00 \pm 1.19$  &         ...        &  0 \\
DES\,J220328.27$-$462809.5  &  330.86780  & $ -46.46932 $ &  21.53  &  21.11  &  57980.9  &    4.0  &  \phs$207.1 \pm 5.5$  &         ...       &         ...        &  0 \\
DES\,J220328.29$-$462639.1  &  330.86788  & $ -46.44420 $ &  17.36  &  16.37  &  57311.3  &   97.6  &   \phs$26.8 \pm 1.2$  &  $6.59 \pm 0.33$  &         ...        &  0 \\
                            &  330.86788  & $ -46.44420 $ &  17.36  &  16.37  &  57980.9  &  161.7  &   \phs$27.2 \pm 1.0$  &  $6.20 \pm 0.32$  &         ...        &  0 \\
                            &  330.86788  & $ -46.44420 $ &  17.36  &  16.37  &  58363.6  &   74.5  &   \phs$28.4 \pm 1.0$  &         ...       &         ...        &  0 \\
DES\,J220329.50$-$461651.5  &  330.87290  & $ -46.28096 $ &  19.28  &  19.02  &  57284.1  &    9.1  &     $-102.9 \pm 2.8$  &         ...       &         ...        &  0 \\
                            &  330.87290  & $ -46.28096 $ &  19.28  &  19.02  &  57630.5  &   12.0  &     $-121.0 \pm 3.9$  &         ...       &         ...        &  0 \\
DES\,J220330.02$-$463132.8  &  330.87509  & $ -46.52577 $ &  20.97  &  20.58  &  57282.6  &    6.9  &   \phs$74.1 \pm 2.2$  &  $4.63 \pm 0.96$  &         ...        &  0 \\
DES\,J220331.60$-$463218.5  &  330.88165  & $ -46.53847 $ &  19.41  &  19.06  &  57282.6  &   23.0  &     $-179.9 \pm 1.3$  &  $2.75 \pm 0.36$  &         ...        &  0 \\
                            &  330.88165  & $ -46.53847 $ &  19.41  &  19.06  &  57634.4  &    7.6  &     $-181.1 \pm 2.6$  &  $3.54 \pm 0.81$  &         ...        &  0 \\
                            &  330.88165  & $ -46.53847 $ &  19.41  &  19.06  &  58363.6  &    9.6  &     $-180.5 \pm 2.1$  &         ...       &         ...        &  0 \\
DES\,J220331.94$-$463147.3  &  330.88308  & $ -46.52979 $ &  20.83  &  20.31  &  57282.6  &    8.8  &  \phs$111.3 \pm 2.2$  &         ...       &         ...        &  0 \\
DES\,J220333.98$-$461558.5  &  330.89157  & $ -46.26625 $ &  19.18  &  18.59  &  57284.1  &   11.0  &   \phs$46.1 \pm 2.0$  &         ...       &         ...        &  0 \\
                            &  330.89157  & $ -46.26625 $ &  19.18  &  18.59  &  57630.5  &   16.6  &   \phs$46.2 \pm 1.3$  &  $6.06 \pm 0.48$  &         ...        &  0 \\
DES\,J220334.56$-$461717.1  &  330.89399  & $ -46.28808 $ &  18.73  &  18.01  &  57284.1  &   25.3  &   \phs$31.7 \pm 1.3$  &         ...       &         ...        &  0 \\
                            &  330.89399  & $ -46.28808 $ &  18.73  &  18.01  &  57630.5  &   30.5  &   \phs$32.3 \pm 1.1$  &         ...       &         ...        &  0 \\
DES\,J220334.66$-$461651.0  &  330.89443  & $ -46.28083 $ &  20.55  &  20.00  &  57284.1  &    5.5  &  \phs$217.6 \pm 5.7$  &         ...       &         ...        &  0 \\
                            &  330.89443  & $ -46.28083 $ &  20.55  &  20.00  &  57630.5  &    6.7  &  \phs$199.7 \pm 2.2$  &  $5.67 \pm 1.02$  &         ...        &  0 \\
DES\,J220334.94$-$461900.4  &  330.89558  & $ -46.31677 $ &  19.73  &  19.22  &  57284.1  &   10.1  &   \phs$60.2 \pm 4.7$  &  $5.48 \pm 1.23$  &         ...        &  0 \\
                            &  330.89558  & $ -46.31677 $ &  19.73  &  19.22  &  57630.5  &   12.5  &   \phs$31.5 \pm 1.6$  &  $4.06 \pm 0.47$  &         ...        &  0 \\
DES\,J220336.21$-$462534.5  &  330.90087  & $ -46.42624 $ &  19.73  &  19.36  &  57980.9  &   18.1  &  \phs$235.0 \pm 1.4$  &  $1.59 \pm 0.36$  &         ...        &  0 \\
                            &  330.90087  & $ -46.42624 $ &  19.73  &  19.36  &  58363.6  &    5.6  &  \phs$229.4 \pm 7.3$  &         ...       &         ...        &  0 \\
DES\,J220336.91$-$463003.7  &  330.90378  & $ -46.50102 $ &  17.96  &  17.41  &  57980.9  &   80.0  &      $-82.9 \pm 1.0$  &  $5.83 \pm 0.33$  &         ...        &  0 \\
                            &  330.90378  & $ -46.50102 $ &  17.96  &  17.41  &  58363.6  &   33.7  &      $-82.5 \pm 1.1$  &  $5.68 \pm 0.37$  &         ...        &  0 \\
DES\,J220337.18$-$462814.1  &  330.90492  & $ -46.47057 $ &  18.73  &  18.26  &  57980.9  &   45.7  &       $-5.3 \pm 1.0$  &  $3.30 \pm 0.34$  &         ...        &  0 \\
DES\,J220338.48$-$461852.7  &  330.91032  & $ -46.31465 $ &  20.26  &  19.63  &  57284.1  &    7.3  &    \phs$1.8 \pm 2.3$  &  $6.46 \pm 0.93$  &         ...        &  0 \\
                            &  330.91032  & $ -46.31465 $ &  20.26  &  19.63  &  57630.5  &    9.3  &       $-1.5 \pm 2.0$  &  $7.27 \pm 0.83$  &         ...        &  0 \\
DES\,J220339.17$-$461240.7  &  330.91322  & $ -46.21132 $ &  18.94  &  18.46  &  57284.1  &   16.8  &    \phs$0.3 \pm 3.8$  &  $4.50 \pm 0.52$  &         ...        &  0 \\
                            &  330.91322  & $ -46.21132 $ &  18.94  &  18.46  &  57630.5  &   20.8  &    \phs$5.7 \pm 2.7$  &  $4.40 \pm 0.53$  &         ...        &  0 \\
DES\,J220341.29$-$462759.5  &  330.92203  & $ -46.46654 $ &  19.11  &  19.16  &  57311.3  &   12.7  &     $-106.9 \pm 1.9$  &         ...       &         ...        &  1 \\
                            &  330.92203  & $ -46.46654 $ &  19.11  &  19.16  &  57980.9  &   19.4  &     $-107.2 \pm 1.4$  &         ...       &         ...        &  1 \\
                            &  330.92203  & $ -46.46654 $ &  19.11  &  19.16  &  58363.6  &    7.1  &     $-111.9 \pm 2.7$  &         ...       &         ...        &  1 \\
DES\,J220342.72$-$462623.0  &  330.92800  & $ -46.43971 $ &  17.17  &  16.42  &  57282.6  &  140.7  &       $-4.2 \pm 1.2$  &  $6.21 \pm 0.32$  &         ...        &  0 \\
                            &  330.92800  & $ -46.43971 $ &  17.17  &  16.42  &  57634.4  &   67.7  &       $-7.2 \pm 1.0$  &         ...       &         ...        &  0 \\
                            &  330.92800  & $ -46.43971 $ &  17.17  &  16.42  &  57980.9  &  139.5  &       $-7.9 \pm 1.0$  &  $5.53 \pm 0.32$  &         ...        &  0 \\
                            &  330.92800  & $ -46.43971 $ &  17.17  &  16.42  &  58339.5  &   95.4  &       $-8.5 \pm 1.0$  &  $6.21 \pm 0.33$  &         ...        &  0 \\
                            &  330.92800  & $ -46.43971 $ &  17.17  &  16.42  &  58363.6  &   64.7  &       $-7.7 \pm 1.0$  &  $6.00 \pm 0.33$  &         ...        &  0 \\
DES\,J220342.76$-$462536.5  &  330.92816  & $ -46.42681 $ &  19.55  &  19.27  &  57311.3  &   11.9  &     $-109.8 \pm 2.1$  &  $1.63 \pm 0.47$  &         ...        &  0 \\
DES\,J220343.10$-$463136.1  &  330.92957  & $ -46.52670 $ &  21.12  &  20.70  &  57282.6  &    5.4  &     $-111.2 \pm 2.0$  &         ...       &         ...        &  1 \\
DES\,J220343.10$-$462804.6  &  330.92959  & $ -46.46793 $ &  20.55  &  20.06  &  57311.3  &    7.6  &   \phs$94.3 \pm 2.3$  &         ...       &         ...        &  0 \\
                            &  330.92959  & $ -46.46793 $ &  20.55  &  20.06  &  57634.4  &    4.3  &  \phs$102.8 \pm 2.9$  &         ...       &         ...        &  0 \\
                            &  330.92959  & $ -46.46793 $ &  20.55  &  20.06  &  58363.6  &    4.3  &   \phs$85.7 \pm 7.6$  &         ...       &         ...        &  0 \\
DES\,J220346.72$-$462240.4  &  330.94468  & $ -46.37789 $ &  19.17  &  18.24  &  58339.5  &   33.5  &  \phs$118.1 \pm 1.1$  &  $5.70 \pm 0.38$  &         ...        &  0 \\
DES\,J220347.66$-$462821.3  &  330.94859  & $ -46.47258 $ &  18.94  &  18.69  &  57282.6  &   31.1  &     $-226.4 \pm 1.4$  &         ...       &         ...        &  0 \\
                            &  330.94859  & $ -46.47258 $ &  18.94  &  18.69  &  57634.4  &   13.7  &     $-225.9 \pm 1.5$  &  $0.80 \pm 0.37$  &         ...        &  0 \\
DES\,J220348.10$-$462759.4  &  330.95043  & $ -46.46650 $ &  19.61  &  18.75  &  57311.3  &   25.3  &      $-14.9 \pm 1.5$  &  $6.34 \pm 0.47$  &         ...        &  0 \\
DES\,J220349.20$-$462957.2  &  330.95499  & $ -46.49923 $ &  21.36  &  20.91  &  57980.9  &    6.3  &      $-97.0 \pm 2.4$  &         ...       &         ...        &  0 \\
DES\,J220349.36$-$462210.5  &  330.95566  & $ -46.36958 $ &  20.02  &  19.50  &  57311.3  &   10.7  &   \phs$19.0 \pm 1.7$  &  $6.13 \pm 0.58$  &         ...        &  0 \\
                            &  330.95566  & $ -46.36958 $ &  20.02  &  19.50  &  58339.5  &   13.6  &   \phs$20.1 \pm 1.6$  &  $5.49 \pm 0.78$  &         ...        &  0 \\
DES\,J220349.47$-$463102.7  &  330.95611  & $ -46.51743 $ &  18.63  &  17.86  &  58363.6  &   27.9  &   \phs$38.5 \pm 1.2$  &  $5.54 \pm 0.39$  &         ...        &  0 \\
DES\,J220349.72$-$463050.8  &  330.95718  & $ -46.51412 $ &  20.62  &  20.30  &  57282.6  &    8.1  &  \phs$174.1 \pm 2.2$  &  $3.18 \pm 0.71$  &         ...        &  0 \\
DES\,J220349.73$-$463314.6  &  330.95722  & $ -46.55405 $ &  16.70  &  15.78  &  58363.6  &   90.8  &       $-4.3 \pm 1.0$  &  $6.47 \pm 0.33$  &         ...        &  0 \\
DES\,J220351.08$-$462552.7  &  330.96283  & $ -46.43130 $ &  21.61  &  20.95  &  57282.6  &    6.9  &   \phs$14.1 \pm 2.6$  &         ...       &         ...        &  0 \\
DES\,J220351.24$-$461711.1  &  330.96351  & $ -46.28641 $ &  20.92  &  19.95  &  57284.1  &    5.9  &   \phs$25.6 \pm 4.6$  &  $4.48 \pm 0.84$  &         ...        &  0 \\
                            &  330.96351  & $ -46.28641 $ &  20.92  &  19.95  &  57630.5  &    8.6  &   \phs$22.1 \pm 1.8$  &  $4.85 \pm 0.69$  &         ...        &  0 \\
DES\,J220351.54$-$461441.7  &  330.96476  & $ -46.24492 $ &  20.93  &  20.24  &  57284.1  &    4.5  &      $-28.3 \pm 2.8$  &  $5.53 \pm 1.92$  &         ...        &  0 \\
                            &  330.96476  & $ -46.24492 $ &  20.93  &  20.24  &  57630.5  &    6.7  &      $-29.6 \pm 2.5$  &         ...       &         ...        &  0 \\
DES\,J220352.01$-$462446.5  &  330.96671  & $ -46.41291 $ &  19.42  &  18.88  &  57282.6  &   32.2  &     $-109.3 \pm 1.3$  &  $1.73 \pm 0.37$  &  $-2.88 \pm 0.24$  &  1 \\
                            &  330.96671  & $ -46.41291 $ &  19.42  &  18.88  &  57311.3  &   19.3  &     $-117.8 \pm 1.3$  &         ...       &         ...        &  1 \\
                            &  330.96671  & $ -46.41291 $ &  19.42  &  18.88  &  57634.4  &   13.2  &     $-110.2 \pm 1.5$  &  $1.45 \pm 0.42$  &  $-3.07 \pm 0.32$  &  1 \\
                            &  330.96671  & $ -46.41291 $ &  19.42  &  18.88  &  57980.9  &   31.9  &     $-107.8 \pm 1.1$  &  $1.67 \pm 0.33$  &  $-2.92 \pm 0.22$  &  1 \\
                            &  330.96671  & $ -46.41291 $ &  19.42  &  18.88  &  58339.5  &   23.4  &     $-107.9 \pm 1.2$  &  $1.43 \pm 0.47$  &  $-3.09 \pm 0.36$  &  1 \\
DES\,J220352.37$-$462540.7  &  330.96821  & $ -46.42797 $ &  21.35  &  20.92  &  57282.6  &    6.2  &     $-113.1 \pm 3.5$  &         ...       &         ...        &  1 \\
                            &  330.96821  & $ -46.42797 $ &  21.35  &  20.92  &  57980.9  &    5.6  &     $-105.1 \pm 6.4$  &         ...       &         ...        &  1 \\
                            &  330.96821  & $ -46.42797 $ &  21.35  &  20.92  &  58339.5  &    4.2  &     $-106.8 \pm 3.0$  &  $3.47 \pm 1.04$  &  $-1.55 \pm 0.51$  &  1 \\
DES\,J220355.46$-$461539.5  &  330.98110  & $ -46.26098 $ &  20.95  &  20.50  &  57630.5  &    4.8  &     $-111.4 \pm 3.3$  &  $2.10 \pm 0.52$  &  $-2.36 \pm 0.30$  &  1 \\
DES\,J220355.93$-$462209.6  &  330.98304  & $ -46.36932 $ &  21.21  &  20.48  &  58339.5  &    6.1  &   \phs$11.4 \pm 2.6$  &  $5.43 \pm 1.32$  &         ...        &  0 \\
DES\,J220355.95$-$462508.1  &  330.98312  & $ -46.41891 $ &  19.20  &  18.92  &  57282.6  &   26.9  &   \phs$29.8 \pm 1.3$  &  $2.79 \pm 0.35$  &         ...        &  0 \\
                            &  330.98312  & $ -46.41891 $ &  19.20  &  18.92  &  57634.4  &    9.9  &   \phs$31.7 \pm 1.7$  &         ...       &         ...        &  0 \\
                            &  330.98312  & $ -46.41891 $ &  19.20  &  18.92  &  57980.9  &   29.1  &   \phs$31.2 \pm 1.2$  &  $2.15 \pm 0.35$  &         ...        &  0 \\
                            &  330.98312  & $ -46.41891 $ &  19.20  &  18.92  &  58339.5  &   20.0  &   \phs$33.5 \pm 1.3$  &         ...       &         ...        &  0 \\
DES\,J220356.00$-$462641.6  &  330.98334  & $ -46.44490 $ &  20.11  &  19.18  &  57980.9  &   29.4  &      $-56.3 \pm 1.2$  &  $5.99 \pm 0.38$  &         ...        &  0 \\
                            &  330.98334  & $ -46.44490 $ &  20.11  &  19.18  &  58339.5  &   20.6  &      $-55.2 \pm 1.3$  &  $6.41 \pm 0.45$  &         ...        &  0 \\
DES\,J220357.02$-$462800.2  &  330.98758  & $ -46.46671 $ &  21.89  &  21.29  &  57282.6  &    4.4  &   \phs$21.9 \pm 4.9$  &         ...       &         ...        &  0 \\
DES\,J220357.07$-$462829.9  &  330.98779  & $ -46.47498 $ &  20.90  &  20.44  &  57282.6  &    7.4  &     $-113.8 \pm 1.8$  &         ...       &         ...        &  1 \\
                            &  330.98779  & $ -46.47498 $ &  20.90  &  20.44  &  57311.3  &    6.5  &     $-109.7 \pm 4.5$  &         ...       &         ...        &  1 \\
DES\,J220357.72$-$462603.6  &  330.99048  & $ -46.43434 $ &  19.67  &  19.13  &  57282.6  &   26.1  &     $-112.5 \pm 1.4$  &         ...       &         ...        &  1 \\
                            &  330.99048  & $ -46.43434 $ &  19.67  &  19.13  &  57634.4  &   10.6  &     $-109.2 \pm 1.7$  &  $1.92 \pm 0.52$  &  $-2.72 \pm 0.31$  &  1 \\
                            &  330.99048  & $ -46.43434 $ &  19.67  &  19.13  &  57980.9  &   29.4  &     $-110.0 \pm 1.1$  &  $1.85 \pm 0.36$  &  $-2.76 \pm 0.22$  &  1 \\
                            &  330.99048  & $ -46.43434 $ &  19.67  &  19.13  &  58339.5  &   19.9  &     $-108.7 \pm 1.2$  &  $1.83 \pm 0.33$  &  $-2.77 \pm 0.21$  &  1 \\
DES\,J220358.17$-$463020.3  &  330.99236  & $ -46.50563 $ &  19.49  &  18.57  &  57311.3  &   30.3  &   \phs$32.6 \pm 1.3$  &  $6.55 \pm 0.39$  &         ...        &  0 \\
                            &  330.99236  & $ -46.50563 $ &  19.49  &  18.57  &  58363.6  &   16.3  &   \phs$32.8 \pm 1.4$  &  $6.46 \pm 0.51$  &         ...        &  0 \\
DES\,J220358.30$-$462525.9  &  330.99291  & $ -46.42386 $ &  19.86  &  19.62  &  57980.9  &   15.1  &     $-171.7 \pm 1.2$  &  $2.27 \pm 0.51$  &         ...        &  0 \\
DES\,J220358.43$-$462751.3  &  330.99344  & $ -46.46424 $ &  18.99  &  18.15  &  57282.6  &   52.1  &      $-87.1 \pm 1.2$  &  $5.71 \pm 0.34$  &         ...        &  0 \\
                            &  330.99344  & $ -46.46424 $ &  18.99  &  18.15  &  57634.4  &   23.2  &      $-85.1 \pm 1.3$  &         ...       &         ...        &  0 \\
DES\,J220359.07$-$462030.7  &  330.99612  & $ -46.34186 $ &  18.71  &  18.22  &  57284.1  &   23.2  &      $-88.7 \pm 1.4$  &  $5.55 \pm 0.41$  &         ...        &  0 \\
                            &  330.99612  & $ -46.34186 $ &  18.71  &  18.22  &  57630.5  &   25.9  &      $-90.1 \pm 1.2$  &  $5.24 \pm 0.39$  &         ...        &  0 \\
DES\,J220400.12$-$462529.0  &  331.00048  & $ -46.42472 $ &  19.92  &  19.28  &  58339.5  &   18.0  &     $-110.9 \pm 1.3$  &  $2.66 \pm 0.42$  &         ...        &  0 \\
DES\,J220400.61$-$461810.2  &  331.00256  & $ -46.30282 $ &  19.59  &  19.06  &  57284.1  &   12.4  &      $-18.2 \pm 1.7$  &  $5.23 \pm 0.59$  &         ...        &  0 \\
DES\,J220401.91$-$461502.7  &  331.00795  & $ -46.25074 $ &  19.21  &  18.68  &  57284.1  &   16.2  &   \phs$52.4 \pm 1.7$  &  $5.83 \pm 0.52$  &         ...        &  0 \\
                            &  331.00795  & $ -46.25074 $ &  19.21  &  18.68  &  57630.5  &   19.2  &   \phs$56.2 \pm 1.2$  &  $5.76 \pm 0.47$  &         ...        &  0 \\
DES\,J220402.83$-$462830.7  &  331.01180  & $ -46.47520 $ &  20.61  &  20.06  &  57282.6  &   11.2  &     $-109.7 \pm 2.9$  &         ...       &         ...        &  0 \\
                            &  331.01180  & $ -46.47520 $ &  20.61  &  20.06  &  57311.3  &    8.2  &     $-105.9 \pm 4.9$  &         ...       &         ...        &  0 \\
                            &  331.01180  & $ -46.47520 $ &  20.61  &  20.06  &  57980.9  &   12.5  &     $-109.2 \pm 1.9$  &  $4.73 \pm 0.73$  &         ...        &  0 \\
DES\,J220403.26$-$462403.3  &  331.01359  & $ -46.40092 $ &  18.59  &  17.93  &  57311.3  &   38.9  &       $-3.7 \pm 1.2$  &  $6.45 \pm 0.36$  &         ...        &  0 \\
                            &  331.01359  & $ -46.40092 $ &  18.59  &  17.93  &  58339.5  &   42.0  &       $-4.4 \pm 1.0$  &  $5.68 \pm 0.35$  &         ...        &  0 \\
DES\,J220403.28$-$462520.0  &  331.01366  & $ -46.42222 $ &  21.12  &  20.67  &  57282.6  &    7.7  &     $-105.0 \pm 4.0$  &  $2.47 \pm 0.67$  &  $-2.12 \pm 0.36$  &  1 \\
                            &  331.01366  & $ -46.42222 $ &  21.12  &  20.67  &  57311.3  &    5.0  &     $-117.4 \pm 3.3$  &         ...       &         ...        &  1 \\
                            &  331.01366  & $ -46.42222 $ &  21.12  &  20.67  &  57980.9  &    7.1  &     $-115.4 \pm 2.3$  &         ...       &         ...        &  1 \\
                            &  331.01366  & $ -46.42222 $ &  21.12  &  20.67  &  58339.5  &    5.4  &     $-112.4 \pm 3.4$  &         ...       &         ...        &  1 \\
DES\,J220405.91$-$462231.3  &  331.02461  & $ -46.37535 $ &  18.19  &  17.55  &  57282.6  &   71.2  &   \phs$44.8 \pm 1.2$  &  $6.16 \pm 0.33$  &         ...        &  0 \\
                            &  331.02461  & $ -46.37535 $ &  18.19  &  17.55  &  57634.4  &   30.3  &   \phs$45.1 \pm 1.1$  &  $6.10 \pm 0.38$  &         ...        &  0 \\
                            &  331.02461  & $ -46.37535 $ &  18.19  &  17.55  &  58339.5  &   52.6  &   \phs$45.6 \pm 1.0$  &  $5.78 \pm 0.34$  &         ...        &  0 \\
DES\,J220406.24$-$462559.6  &  331.02601  & $ -46.43321 $ &  19.74  &  18.91  &  57282.6  &   31.3  &      $-49.4 \pm 1.3$  &         ...       &         ...        &  0 \\
                            &  331.02601  & $ -46.43321 $ &  19.74  &  18.91  &  57634.4  &   12.5  &      $-49.4 \pm 1.6$  &  $5.27 \pm 0.55$  &         ...        &  0 \\
DES\,J220406.57$-$462640.3  &  331.02736  & $ -46.44452 $ &  20.91  &  20.40  &  57980.9  &   10.1  &   \phs$94.2 \pm 3.3$  &  $1.99 \pm 0.44$  &         ...        &  0 \\
                            &  331.02736  & $ -46.44452 $ &  20.91  &  20.40  &  58339.5  &    7.1  &   \phs$92.9 \pm 3.4$  &  $3.71 \pm 0.67$  &         ...        &  0 \\
DES\,J220408.41$-$462656.9  &  331.03505  & $ -46.44915 $ &  18.66  &  18.37  &  57980.9  &   45.3  &      $-71.5 \pm 1.1$  &  $1.83 \pm 0.35$  &         ...        &  0 \\
                            &  331.03505  & $ -46.44915 $ &  18.66  &  18.37  &  58339.5  &   29.8  &      $-70.3 \pm 1.1$  &  $1.70 \pm 0.35$  &         ...        &  0 \\
DES\,J220408.88$-$462416.7  &  331.03698  & $ -46.40463 $ &  18.91  &  18.08  &  58339.5  &   38.8  &      $-24.0 \pm 1.1$  &  $5.86 \pm 0.35$  &         ...        &  0 \\
DES\,J220408.90$-$461927.5  &  331.03708  & $ -46.32431 $ &  20.88  &  19.93  &  57284.1  &    7.5  &   \phs$32.7 \pm 3.5$  &  $5.33 \pm 1.10$  &         ...        &  0 \\
                            &  331.03708  & $ -46.32431 $ &  20.88  &  19.93  &  57630.5  &    9.5  &   \phs$29.5 \pm 1.9$  &  $6.12 \pm 1.07$  &         ...        &  0 \\
DES\,J220409.31$-$462339.3  &  331.03881  & $ -46.39425 $ &  19.29  &  18.53  &  57980.9  &   48.1  &      $-84.3 \pm 1.1$  &  $6.01 \pm 0.34$  &         ...        &  0 \\
DES\,J220409.98$-$462102.2  &  331.04158  & $ -46.35061 $ &  18.19  &  17.49  &  57284.1  &   40.6  &     $-107.6 \pm 1.2$  &  $2.63 \pm 0.33$  &  $-2.67 \pm 0.16$  &  1 \\
                            &  331.04158  & $ -46.35061 $ &  18.19  &  17.49  &  57630.5  &   43.1  &     $-108.2 \pm 1.0$  &  $2.28 \pm 0.35$  &  $-2.84 \pm 0.18$  &  1 \\
DES\,J220410.77$-$463202.5  &  331.04486  & $ -46.53403 $ &  17.36  &  16.54  &  57311.3  &   99.0  &   \phs$58.8 \pm 1.2$  &  $6.33 \pm 0.33$  &         ...        &  0 \\
DES\,J220410.93$-$463019.8  &  331.04555  & $ -46.50549 $ &  19.53  &  19.07  &  57311.3  &   19.3  &       $-3.6 \pm 1.4$  &  $3.69 \pm 0.44$  &         ...        &  0 \\
                            &  331.04555  & $ -46.50549 $ &  19.53  &  19.07  &  58363.6  &    9.0  &       $-5.4 \pm 1.6$  &  $3.84 \pm 0.65$  &         ...        &  0 \\
DES\,J220412.35$-$462543.1  &  331.05145  & $ -46.42863 $ &  20.90  &  20.47  &  57282.6  &    7.7  &   \phs$57.6 \pm 2.8$  &         ...       &         ...        &  0 \\
                            &  331.05145  & $ -46.42863 $ &  20.90  &  20.47  &  57311.3  &    5.8  &   \phs$62.6 \pm 6.4$  &  $3.76 \pm 0.71$  &         ...        &  0 \\
DES\,J220413.66$-$461743.7  &  331.05692  & $ -46.29547 $ &  19.00  &  18.61  &  57284.1  &   17.4  &      $-19.6 \pm 1.5$  &  $4.10 \pm 0.45$  &         ...        &  0 \\
                            &  331.05692  & $ -46.29547 $ &  19.00  &  18.61  &  57630.5  &   19.8  &      $-20.6 \pm 1.3$  &  $4.13 \pm 0.39$  &         ...        &  0 \\
DES\,J220415.84$-$462454.9  &  331.06599  & $ -46.41524 $ &  18.33  &  17.71  &  57282.6  &   32.9  &       $-4.7 \pm 1.3$  &  $5.18 \pm 0.39$  &         ...        &  0 \\
                            &  331.06599  & $ -46.41524 $ &  18.33  &  17.71  &  57634.4  &   25.3  &       $-3.5 \pm 1.1$  &  $5.59 \pm 0.40$  &         ...        &  0 \\
                            &  331.06599  & $ -46.41524 $ &  18.33  &  17.71  &  57980.9  &   77.0  &       $-3.1 \pm 1.0$  &  $5.52 \pm 0.33$  &         ...        &  0 \\
DES\,J220416.29$-$462822.3  &  331.06788  & $ -46.47285 $ &  18.57  &  18.34  &  57282.6  &   35.0  &    \phs$4.7 \pm 1.3$  &  $1.46 \pm 0.39$  &         ...        &  0 \\
                            &  331.06788  & $ -46.47285 $ &  18.57  &  18.34  &  57634.4  &   14.6  &    \phs$5.0 \pm 1.4$  &  $1.97 \pm 0.36$  &         ...        &  0 \\
DES\,J220416.46$-$462225.3  &  331.06858  & $ -46.37369 $ &  20.54  &  20.01  &  57284.1  &    5.8  &     $-106.0 \pm 2.5$  &  $3.77 \pm 0.78$  &  $-1.61 \pm 0.37$  &  1 \\
                            &  331.06858  & $ -46.37369 $ &  20.54  &  20.01  &  57630.5  &    6.2  &     $-110.2 \pm 2.2$  &         ...       &         ...        &  1 \\
                            &  331.06858  & $ -46.37369 $ &  20.54  &  20.01  &  58339.5  &   10.5  &     $-111.0 \pm 1.6$  &  $2.90 \pm 0.58$  &  $-2.03 \pm 0.29$  &  1 \\
DES\,J220416.72$-$462432.6  &  331.06968  & $ -46.40907 $ &  21.56  &  21.12  &  57980.9  &    5.3  &     $-112.2 \pm 2.0$  &         ...       &         ...        &  1 \\
DES\,J220416.80$-$463432.1  &  331.07002  & $ -46.57559 $ &  19.18  &  18.63  &  57311.3  &   25.9  &  \phs$179.7 \pm 1.4$  &  $6.35 \pm 0.44$  &         ...        &  0 \\
DES\,J220417.31$-$462302.3  &  331.07213  & $ -46.38397 $ &  19.52  &  19.25  &  57980.9  &   26.0  &  \phs$131.6 \pm 1.2$  &  $2.46 \pm 0.42$  &         ...        &  0 \\
                            &  331.07213  & $ -46.38397 $ &  19.52  &  19.25  &  58339.5  &   16.6  &  \phs$135.6 \pm 1.4$  &  $2.27 \pm 0.47$  &         ...        &  0 \\
DES\,J220418.14$-$463252.1  &  331.07559  & $ -46.54781 $ &  19.87  &  19.33  &  57311.3  &   16.7  &     $-107.2 \pm 1.6$  &         ...       &         ...        &  1 \\
                            &  331.07559  & $ -46.54781 $ &  19.87  &  19.33  &  57981.0  &    7.4  &     $-108.7 \pm 2.5$  &         ...       &         ...        &  1 \\
DES\,J220418.47$-$463534.0  &  331.07697  & $ -46.59278 $ &  21.12  &  20.70  &  57311.3  &    4.5  &      $-58.2 \pm 5.7$  &         ...       &         ...        &  0 \\
DES\,J220419.17$-$462831.5  &  331.07988  & $ -46.47541 $ &  18.49  &  17.91  &  57311.3  &   45.5  &      $-53.5 \pm 1.3$  &  $4.26 \pm 0.35$  &         ...        &  0 \\
DES\,J220419.89$-$462444.5  &  331.08287  & $ -46.41236 $ &  21.04  &  20.71  &  57980.9  &    6.9  &  \phs$178.8 \pm 2.2$  &         ...       &         ...        &  0 \\
DES\,J220420.12$-$462341.3  &  331.08385  & $ -46.39481 $ &  19.20  &  19.33  &  57284.1  &    6.8  &     $-110.5 \pm 2.6$  &         ...       &         ...        &  1 \\
                            &  331.08385  & $ -46.39481 $ &  19.20  &  19.33  &  57630.5  &    7.5  &     $-104.8 \pm 3.2$  &         ...       &         ...        &  1 \\
                            &  331.08385  & $ -46.39481 $ &  19.20  &  19.33  &  57980.9  &   18.8  &     $-113.9 \pm 1.7$  &         ...       &         ...        &  1 \\
                            &  331.08385  & $ -46.39481 $ &  19.20  &  19.33  &  58339.5  &   12.4  &     $-106.9 \pm 2.2$  &         ...       &         ...        &  1 \\
DES\,J220420.84$-$463621.2  &  331.08682  & $ -46.60589 $ &  17.73  &  17.00  &  57311.3  &   68.5  &       $-6.4 \pm 1.2$  &  $6.60 \pm 0.33$  &         ...        &  0 \\
                            &  331.08682  & $ -46.60589 $ &  17.73  &  17.00  &  57981.0  &   34.7  &       $-9.9 \pm 1.0$  &  $7.94 \pm 0.37$  &         ...        &  0 \\
DES\,J220422.11$-$461835.5  &  331.09212  & $ -46.30985 $ &  18.19  &  17.60  &  57284.1  &   35.8  &      $-34.4 \pm 1.3$  &  $5.47 \pm 0.36$  &         ...        &  0 \\
                            &  331.09212  & $ -46.30985 $ &  18.19  &  17.60  &  57630.5  &   38.9  &      $-34.3 \pm 1.0$  &  $5.67 \pm 0.37$  &         ...        &  0 \\
DES\,J220423.14$-$463346.9  &  331.09642  & $ -46.56303 $ &  18.54  &  18.05  &  57981.0  &   18.9  &      $-52.6 \pm 1.2$  &  $3.49 \pm 0.41$  &         ...        &  0 \\
DES\,J220423.45$-$462703.4  &  331.09769  & $ -46.45093 $ &  19.48  &  19.07  &  58339.5  &   17.9  &    \phs$1.2 \pm 1.3$  &  $4.05 \pm 0.45$  &         ...        &  0 \\
DES\,J220423.91$-$463702.5  &  331.09961  & $ -46.61736 $ &  17.55  &  16.76  &  57981.0  &   42.8  &     $-108.6 \pm 1.0$  &  $3.07 \pm 0.35$  &  $-2.62 \pm 0.16$  &  1 \\
DES\,J220425.07$-$463041.4  &  331.10444  & $ -46.51150 $ &  19.06  &  18.33  &  57311.3  &   36.3  &       $-2.5 \pm 1.3$  &  $5.69 \pm 0.37$  &         ...        &  0 \\
DES\,J220425.34$-$463015.2  &  331.10560  & $ -46.50421 $ &  21.14  &  20.65  &  57311.3  &    6.2  &      $-33.1 \pm 3.1$  &         ...       &         ...        &  0 \\
DES\,J220426.35$-$462229.9  &  331.10979  & $ -46.37496 $ &  20.91  &  20.02  &  58339.5  &   11.5  &   \phs$40.2 \pm 1.8$  &  $4.75 \pm 0.62$  &         ...        &  0 \\
DES\,J220427.66$-$462839.5  &  331.11527  & $ -46.47764 $ &  20.95  &  20.49  &  57311.3  &    6.3  &     $-109.6 \pm 2.5$  &         ...       &         ...        &  1 \\
                            &  331.11527  & $ -46.47764 $ &  20.95  &  20.49  &  57980.9  &    7.8  &     $-109.3 \pm 2.1$  &         ...       &         ...        &  1 \\
DES\,J220428.42$-$463037.3  &  331.11841  & $ -46.51037 $ &  20.05  &  19.85  &  57311.3  &    8.9  &  \phs$214.6 \pm 2.6$  &         ...       &         ...        &  0 \\
                            &  331.11841  & $ -46.51037 $ &  20.05  &  19.85  &  57981.0  &    5.0  &     $-110.7 \pm 2.6$  &         ...       &         ...        &  0 \\
DES\,J220428.60$-$461736.1  &  331.11916  & $ -46.29335 $ &  17.72  &  17.01  &  57284.1  &   52.7  &   \phs$45.4 \pm 3.4$  &  $4.17 \pm 0.48$  &         ...        &  0 \\
DES\,J220430.68$-$463138.2  &  331.12785  & $ -46.52728 $ &  21.33  &  20.54  &  57311.3  &    6.8  &   \phs$27.1 \pm 7.1$  &         ...       &         ...        &  0 \\
DES\,J220431.04$-$463448.4  &  331.12935  & $ -46.58010 $ &  17.43  &  16.73  &  57311.3  &   79.9  &       $-1.8 \pm 1.2$  &  $5.51 \pm 0.33$  &         ...        &  0 \\
DES\,J220431.94$-$463529.8  &  331.13308  & $ -46.59161 $ &  18.41  &  17.76  &  57311.3  &   43.4  &      $-54.7 \pm 1.3$  &  $5.96 \pm 0.36$  &         ...        &  0 \\
                            &  331.13308  & $ -46.59161 $ &  18.41  &  17.76  &  57981.0  &   23.1  &      $-56.7 \pm 1.2$  &  $5.57 \pm 0.43$  &         ...        &  0 \\
DES\,J220431.99$-$461929.0  &  331.13329  & $ -46.32473 $ &  18.14  &  17.55  &  57284.1  &   36.2  &      $-49.2 \pm 1.3$  &  $5.98 \pm 0.36$  &         ...        &  0 \\
                            &  331.13329  & $ -46.32473 $ &  18.14  &  17.55  &  57630.5  &   38.7  &      $-48.3 \pm 1.1$  &  $5.57 \pm 0.35$  &         ...        &  0 \\
DES\,J220432.12$-$462231.5  &  331.13383  & $ -46.37542 $ &  19.99  &  19.75  &  57284.1  &    5.4  &     $-167.1 \pm 2.6$  &         ...       &         ...        &  0 \\
                            &  331.13383  & $ -46.37542 $ &  19.99  &  19.75  &  57630.5  &    6.2  &     $-166.6 \pm 3.0$  &  $1.76 \pm 0.40$  &         ...        &  0 \\
                            &  331.13383  & $ -46.37542 $ &  19.99  &  19.75  &  58339.5  &   11.7  &     $-160.4 \pm 1.8$  &  $2.28 \pm 0.46$  &         ...        &  0 \\
DES\,J220432.96$-$463005.9  &  331.13732  & $ -46.50162 $ &  19.75  &  19.15  &  57311.3  &   21.5  &      $-15.3 \pm 1.3$  &  $3.23 \pm 0.43$  &         ...        &  0 \\
DES\,J220433.63$-$463251.1  &  331.14011  & $ -46.54754 $ &  20.99  &  20.61  &  57311.3  &    5.3  &     $-155.1 \pm 4.2$  &         ...       &         ...        &  0 \\
DES\,J220433.75$-$462639.8  &  331.14063  & $ -46.44439 $ &  19.18  &  19.31  &  57980.9  &   15.6  &     $-110.3 \pm 1.7$  &         ...       &         ...        &  1 \\
                            &  331.14063  & $ -46.44439 $ &  19.18  &  19.31  &  57981.0  &    5.2  &     $-121.9 \pm 2.7$  &         ...       &         ...        &  1 \\
                            &  331.14063  & $ -46.44439 $ &  19.18  &  19.31  &  58339.5  &   13.2  &     $-107.4 \pm 1.9$  &         ...       &         ...        &  1 \\
DES\,J220434.10$-$461910.4  &  331.14210  & $ -46.31956 $ &  20.61  &  20.14  &  57284.1  &    5.6  &     $-114.0 \pm 3.4$  &         ...       &         ...        &  1 \\
                            &  331.14210  & $ -46.31956 $ &  20.61  &  20.14  &  57630.5  &    6.4  &     $-110.7 \pm 3.5$  &         ...       &         ...        &  1 \\
DES\,J220435.53$-$463134.1  &  331.14806  & $ -46.52613 $ &  18.87  &  18.75  &  57311.3  &   20.1  &   \phs$10.0 \pm 1.4$  &  $2.45 \pm 0.44$  &         ...        &  0 \\
                            &  331.14806  & $ -46.52613 $ &  18.87  &  18.75  &  57981.0  &    9.4  &    \phs$5.2 \pm 3.9$  &         ...       &         ...        &  0 \\
DES\,J220436.46$-$462423.4  &  331.15193  & $ -46.40650 $ &  19.10  &  18.19  &  57980.9  &   54.2  &    \phs$7.2 \pm 1.0$  &  $6.32 \pm 0.34$  &         ...        &  0 \\
                            &  331.15193  & $ -46.40650 $ &  19.10  &  18.19  &  57981.0  &   17.3  &    \phs$5.1 \pm 1.5$  &  $5.12 \pm 0.45$  &         ...        &  0 \\
DES\,J220437.47$-$461955.0  &  331.15614  & $ -46.33194 $ &  20.45  &  19.99  &  57284.1  &    5.5  &     $-114.3 \pm 2.5$  &         ...       &         ...        &  1 \\
                            &  331.15614  & $ -46.33194 $ &  20.45  &  19.99  &  57630.5  &    7.0  &     $-107.2 \pm 2.1$  &         ...       &         ...        &  1 \\
DES\,J220441.57$-$462244.8  &  331.17320  & $ -46.37911 $ &  17.91  &  17.28  &  58339.5  &   65.8  &     $-160.8 \pm 1.0$  &  $4.06 \pm 0.33$  &         ...        &  0 \\
DES\,J220442.14$-$462553.4  &  331.17559  & $ -46.43151 $ &  19.82  &  19.38  &  57981.0  &    5.6  &   \phs$73.9 \pm 2.0$  &  $3.77 \pm 0.66$  &         ...        &  0 \\
DES\,J220442.40$-$462714.0  &  331.17667  & $ -46.45390 $ &  18.10  &  17.50  &  57981.0  &   25.7  &      $-22.3 \pm 1.2$  &         ...       &         ...        &  0 \\
DES\,J220442.75$-$461942.0  &  331.17811  & $ -46.32832 $ &  19.29  &  18.51  &  57284.1  &   19.5  &   \phs$46.1 \pm 1.4$  &  $6.22 \pm 0.45$  &         ...        &  0 \\
                            &  331.17811  & $ -46.32832 $ &  19.29  &  18.51  &  57630.5  &   22.4  &   \phs$45.2 \pm 1.2$  &  $6.02 \pm 0.43$  &         ...        &  0 \\
DES\,J220445.03$-$462813.8  &  331.18763  & $ -46.47050 $ &  20.16  &  19.40  &  58339.5  &   17.5  &  \phs$151.6 \pm 1.3$  &  $4.28 \pm 0.47$  &         ...        &  0 \\
DES\,J220448.87$-$462539.2  &  331.20362  & $ -46.42755 $ &  20.95  &  20.08  &  58339.5  &   10.8  &      $-21.0 \pm 1.9$  &  $5.74 \pm 0.60$  &         ...        &  0 \\
DES\,J220450.08$-$462952.8  &  331.20869  & $ -46.49800 $ &  18.56  &  17.90  &  57981.0  &   20.9  &      $-42.3 \pm 1.2$  &  $5.77 \pm 0.45$  &         ...        &  0 \\
DES\,J220450.65$-$462928.2  &  331.21103  & $ -46.49116 $ &  19.01  &  18.63  &  57981.0  &   11.8  &       $-6.6 \pm 1.4$  &  $3.66 \pm 0.53$  &         ...        &  0 \\
                            &  331.21103  & $ -46.49116 $ &  19.01  &  18.63  &  58339.5  &   24.5  &       $-7.1 \pm 1.1$  &  $3.72 \pm 0.37$  &         ...        &  0 \\
DES\,J220450.75$-$463514.4  &  331.21144  & $ -46.58735 $ &  18.84  &  18.32  &  57981.0  &   14.6  &   \phs$22.0 \pm 1.2$  &  $5.12 \pm 0.48$  &         ...        &  0 \\
DES\,J220450.86$-$462719.5  &  331.21193  & $ -46.45542 $ &  20.27  &  19.70  &  57981.0  &    4.2  &   \phs$22.6 \pm 3.2$  &         ...       &         ...        &  0 \\
                            &  331.21193  & $ -46.45542 $ &  20.27  &  19.70  &  58339.5  &   12.9  &   \phs$27.0 \pm 1.6$  &  $4.50 \pm 0.54$  &         ...        &  0 \\
DES\,J220451.54$-$462459.0  &  331.21474  & $ -46.41638 $ &  19.57  &  19.33  &  58339.5  &   15.1  &   \phs$88.3 \pm 1.5$  &  $1.73 \pm 0.38$  &         ...        &  0 \\
DES\,J220453.33$-$462851.1  &  331.22220  & $ -46.48086 $ &  20.61  &  20.02  &  58339.5  &    9.7  &   \phs$72.8 \pm 1.8$  &  $5.71 \pm 0.72$  &         ...        &  0 \\
DES\,J220458.78$-$462710.6  &  331.24492  & $ -46.45296 $ &  20.38  &  19.91  &  58339.5  &   10.4  &     $-159.1 \pm 1.9$  &  $2.69 \pm 0.69$  &         ...        &  0 \\
DES\,J220459.55$-$462547.7  &  331.24815  & $ -46.42990 $ &  19.44  &  19.07  &  58339.5  &   18.1  &   \phs$54.7 \pm 1.3$  &  $3.94 \pm 0.46$  &         ...        &  0 \\
DES\,J220505.12$-$462806.7  &  331.27132  & $ -46.46854 $ &  20.53  &  20.09  &  58339.5  &    7.2  &  \phs$149.1 \pm 2.6$  &  $6.04 \pm 0.97$  &         ...        &  0 \\
DES\,J220507.25$-$462815.6  &  331.28019  & $ -46.47099 $ &  18.02  &  17.53  &  58339.5  &   46.4  &      $-17.3 \pm 1.1$  &  $5.45 \pm 0.35$  &         ...        &  0 \\
DES\,J220508.69$-$462408.9  &  331.28623  & $ -46.40248 $ &  20.29  &  19.82  &  58339.5  &   12.5  &     $-111.6 \pm 1.4$  &  $2.14 \pm 0.63$  &  $-2.47 \pm 0.35$  &  1 \\
DES\,J220508.89$-$462743.6  &  331.28702  & $ -46.46210 $ &  18.79  &  18.34  &  58339.5  &   28.8  &   \phs$32.3 \pm 1.1$  &  $2.67 \pm 0.38$  &         ...        &  0 \\
DES\,J000102.48$-$605136.4  &    0.26033  & $ -60.86012 $ &  20.23  &  19.34  &  57981.2  &    7.6  &   \phs$44.6 \pm 7.5$  &  $6.75 \pm 1.15$  &         ...        &  0 \\
DES\,J000105.85$-$605239.1  &    0.27438  & $ -60.87752 $ &  19.44  &  18.91  &  57981.2  &    9.1  &  \phs$107.7 \pm 2.7$  &  $4.95 \pm 0.80$  &         ...        &  0 \\
DES\,J000108.44$-$605359.9  &    0.28516  & $ -60.89998 $ &  19.41  &  18.48  &  57981.2  &   19.1  &  \phs$108.3 \pm 1.3$  &  $6.28 \pm 0.46$  &         ...        &  0 \\
DES\,J000108.59$-$605038.2  &    0.28581  & $ -60.84395 $ &  20.26  &  19.61  &  57981.2  &    4.1  &   \phs$45.0 \pm 4.5$  &         ...       &         ...        &  0 \\
DES\,J000112.27$-$610100.8  &    0.30113  & $ -61.01689 $ &  21.08  &  20.64  &  58340.3  &    6.0  &       $-2.9 \pm 2.2$  &  $4.40 \pm 0.85$  &         ...        &  0 \\
DES\,J000119.59$-$604439.2  &    0.33163  & $ -60.74424 $ &  19.91  &  19.43  &  58339.3  &   13.7  &   \phs$12.4 \pm 1.4$  &  $1.01 \pm 0.50$  &  $-3.32 \pm 0.61$  &  1 \\
                            &    0.33163  & $ -60.74424 $ &  19.91  &  19.43  &  58363.8  &    7.9  &   \phs$25.4 \pm 2.4$  &  $1.15 \pm 0.64$  &  $-3.17 \pm 0.65$  &  1 \\
DES\,J000120.28$-$603918.3  &    0.33449  & $ -60.65508 $ &  17.18  &  16.42  &  58339.3  &   90.0  &   \phs$12.7 \pm 1.0$  &  $6.03 \pm 0.33$  &         ...        &  0 \\
DES\,J000121.36$-$610258.2  &    0.33901  & $ -61.04950 $ &  20.53  &  20.03  &  58340.3  &   10.9  &  \phs$154.2 \pm 1.8$  &  $4.73 \pm 0.60$  &         ...        &  0 \\
DES\,J000122.25$-$605217.5  &    0.34272  & $ -60.87153 $ &  18.54  &  18.09  &  57981.2  &   14.7  &  \phs$115.7 \pm 1.6$  &         ...       &         ...        &  0 \\
DES\,J000124.43$-$605449.8  &    0.35179  & $ -60.91385 $ &  20.25  &  19.39  &  57981.2  &    8.0  &   \phs$62.0 \pm 3.1$  &         ...       &         ...        &  0 \\
DES\,J000127.92$-$603941.9  &    0.36634  & $ -60.66165 $ &  21.48  &  20.73  &  58339.3  &    4.9  &      $-15.6 \pm 3.1$  &  $6.32 \pm 1.11$  &         ...        &  0 \\
DES\,J000129.95$-$610230.1  &    0.37478  & $ -61.04168 $ &  17.93  &  17.26  &  58340.3  &   78.3  &  \phs$213.3 \pm 1.0$  &  $5.57 \pm 0.33$  &         ...        &  0 \\
DES\,J000130.96$-$604233.8  &    0.37900  & $ -60.70940 $ &  20.00  &  19.70  &  58339.3  &   10.6  &   \phs$62.2 \pm 1.8$  &  $2.11 \pm 0.81$  &         ...        &  0 \\
DES\,J000131.89$-$605945.1  &    0.38286  & $ -60.99586 $ &  18.10  &  17.53  &  57981.2  &   31.3  &   \phs$27.4 \pm 1.1$  &  $5.76 \pm 0.39$  &         ...        &  0 \\
DES\,J000132.03$-$604139.4  &    0.38348  & $ -60.69428 $ &  21.13  &  20.72  &  58339.3  &    4.3  &   \phs$31.5 \pm 2.7$  &  $2.71 \pm 0.73$  &         ...        &  0 \\
DES\,J000140.47$-$605439.1  &    0.41863  & $ -60.91086 $ &  19.53  &  19.02  &  57981.2  &    9.5  &   \phs$72.7 \pm 2.1$  &  $6.38 \pm 0.77$  &         ...        &  0 \\
DES\,J000141.19$-$604349.8  &    0.42161  & $ -60.73050 $ &  18.66  &  18.43  &  58339.3  &   24.9  &   \phs$31.6 \pm 1.2$  &  $1.88 \pm 0.35$  &         ...        &  0 \\
DES\,J000142.24$-$603856.3  &    0.42599  & $ -60.64898 $ &  19.56  &  18.93  &  58339.3  &   21.3  &      $-19.3 \pm 1.2$  &  $5.42 \pm 0.44$  &         ...        &  0 \\
DES\,J000142.31$-$610128.2  &    0.42630  & $ -61.02450 $ &  19.97  &  19.62  &  57981.2  &    6.9  &   \phs$83.0 \pm 2.6$  &  $4.51 \pm 0.80$  &         ...        &  0 \\
                            &    0.42630  & $ -61.02450 $ &  19.97  &  19.62  &  58340.3  &   14.4  &   \phs$86.0 \pm 1.4$  &  $4.47 \pm 0.64$  &         ...        &  0 \\
DES\,J000142.89$-$603817.8  &    0.42873  & $ -60.63829 $ &  20.74  &  20.46  &  58339.3  &    5.3  &      $-20.2 \pm 3.0$  &  $2.49 \pm 0.53$  &         ...        &  0 \\
DES\,J000144.29$-$604954.8  &    0.43452  & $ -60.83188 $ &  19.91  &  19.37  &  57981.2  &    4.0  &   \phs$31.7 \pm 7.3$  &         ...       &         ...        &  0 \\
DES\,J000144.47$-$605659.2  &    0.43529  & $ -60.94978 $ &  19.43  &  19.06  &  57981.2  &    9.4  &      $-78.8 \pm 2.5$  &         ...       &         ...        &  0 \\
DES\,J000146.11$-$610254.5  &    0.44214  & $ -61.04846 $ &  20.92  &  20.46  &  58340.3  &    6.6  &   \phs$13.5 \pm 2.3$  &  $0.83 \pm 0.40$  &  $-3.40 \pm 0.72$  &  1 \\
DES\,J000147.09$-$604059.5  &    0.44620  & $ -60.68320 $ &  20.26  &  19.54  &  58339.3  &   14.0  &  \phs$166.4 \pm 1.6$  &  $5.48 \pm 0.76$  &         ...        &  0 \\
DES\,J000149.99$-$604346.9  &    0.45828  & $ -60.72970 $ &  18.35  &  17.77  &  58339.3  &   40.5  &   \phs$53.6 \pm 1.1$  &  $5.90 \pm 0.35$  &         ...        &  0 \\
DES\,J000150.03$-$610113.7  &    0.45846  & $ -61.02047 $ &  19.79  &  19.26  &  57981.2  &    9.4  &  \phs$138.7 \pm 1.9$  &  $4.20 \pm 0.66$  &         ...        &  0 \\
DES\,J000150.26$-$604159.1  &    0.45941  & $ -60.69975 $ &  21.35  &  20.67  &  58339.3  &    4.9  &  \phs$224.7 \pm 6.1$  &         ...       &         ...        &  0 \\
DES\,J000151.52$-$603952.0  &    0.46465  & $ -60.66446 $ &  19.60  &  18.80  &  58339.3  &   24.7  &  \phs$111.8 \pm 1.2$  &  $5.31 \pm 0.40$  &         ...        &  0 \\
DES\,J000154.90$-$603851.1  &    0.47874  & $ -60.64753 $ &  20.29  &  20.12  &  58339.3  &    7.1  &  \phs$136.4 \pm 2.3$  &         ...       &         ...        &  0 \\
DES\,J000155.69$-$610108.5  &    0.48203  & $ -61.01902 $ &  19.01  &  18.01  &  58340.3  &   53.4  &   \phs$60.6 \pm 1.0$  &  $5.89 \pm 0.35$  &         ...        &  0 \\
DES\,J000157.86$-$603752.5  &    0.49107  & $ -60.63124 $ &  21.04  &  20.62  &  58339.3  &    5.5  &   \phs$19.2 \pm 2.8$  &  $0.86 \pm 0.50$  &  $-3.33 \pm 0.83$  &  1 \\
DES\,J000159.19$-$610150.2  &    0.49662  & $ -61.03061 $ &  20.32  &  19.85  &  57981.2  &    5.4  &  \phs$269.8 \pm 2.9$  &         ...       &         ...        &  0 \\
                            &    0.49662  & $ -61.03061 $ &  20.32  &  19.85  &  58340.3  &   13.9  &  \phs$272.6 \pm 1.6$  &  $3.09 \pm 0.60$  &         ...        &  0 \\
DES\,J000201.07$-$604359.2  &    0.50447  & $ -60.73311 $ &  20.15  &  19.57  &  57633.9  &    8.5  &   \phs$34.0 \pm 4.2$  &  $2.32 \pm 0.38$  &         ...        &  0 \\
DES\,J000201.28$-$603946.2  &    0.50532  & $ -60.66284 $ &  18.47  &  18.24  &  58339.3  &   29.6  &      $-46.9 \pm 1.1$  &  $1.88 \pm 0.41$  &         ...        &  0 \\
DES\,J000202.93$-$603736.6  &    0.51221  & $ -60.62684 $ &  19.32  &  18.35  &  58339.3  &   37.6  &   \phs$34.2 \pm 1.1$  &  $5.82 \pm 0.36$  &         ...        &  0 \\
DES\,J000210.80$-$610457.8  &    0.54500  & $ -61.08273 $ &  20.12  &  19.64  &  58340.3  &   17.1  &  \phs$123.3 \pm 1.3$  &  $2.51 \pm 0.49$  &         ...        &  0 \\
                            &    0.54500  & $ -61.08273 $ &  20.12  &  19.64  &  58340.1  &    5.3  &  \phs$124.0 \pm 2.4$  &         ...       &         ...        &  0 \\
DES\,J000211.40$-$604431.6  &    0.54750  & $ -60.74211 $ &  17.97  &  17.43  &  57633.9  &   40.5  &    \phs$3.3 \pm 1.1$  &         ...       &         ...        &  0 \\
DES\,J000212.69$-$604258.2  &    0.55289  & $ -60.71618 $ &  19.80  &  19.21  &  58339.3  &   16.7  &   \phs$53.1 \pm 1.4$  &  $5.09 \pm 0.48$  &         ...        &  0 \\
DES\,J000214.43$-$610026.5  &    0.56011  & $ -61.00737 $ &  20.00  &  19.11  &  58340.3  &   27.2  &   \phs$63.9 \pm 1.2$  &  $6.49 \pm 0.41$  &         ...        &  0 \\
DES\,J000215.97$-$604533.1  &    0.56654  & $ -60.75919 $ &  19.32  &  18.79  &  57633.9  &   14.5  &   \phs$18.3 \pm 1.8$  &  $4.62 \pm 0.61$  &         ...        &  0 \\
DES\,J000216.41$-$610034.7  &    0.56836  & $ -61.00965 $ &  18.07  &  17.53  &  57981.2  &   29.2  &   \phs$44.7 \pm 1.1$  &         ...       &         ...        &  0 \\
                            &    0.56836  & $ -61.00965 $ &  18.07  &  17.53  &  58340.3  &   64.6  &   \phs$41.2 \pm 1.0$  &  $5.63 \pm 0.33$  &         ...        &  0 \\
DES\,J000220.28$-$610512.6  &    0.58449  & $ -61.08682 $ &  19.63  &  18.98  &  58340.3  &   27.9  &  \phs$149.0 \pm 1.2$  &  $6.08 \pm 0.39$  &         ...        &  0 \\
DES\,J000220.28$-$604035.5  &    0.58451  & $ -60.67653 $ &  21.05  &  20.53  &  58339.3  &    5.3  &  \phs$158.8 \pm 2.6$  &  $3.38 \pm 1.30$  &         ...        &  0 \\
DES\,J000222.02$-$605433.1  &    0.59176  & $ -60.90918 $ &  20.93  &  19.94  &  57247.4  &    5.5  &   \phs$44.8 \pm 8.1$  &  $4.35 \pm 1.10$  &         ...        &  0 \\
                            &    0.59176  & $ -60.90918 $ &  20.93  &  19.94  &  57282.3  &    7.0  &   \phs$43.3 \pm 2.9$  &  $5.57 \pm 0.73$  &         ...        &  0 \\
                            &    0.59176  & $ -60.90918 $ &  20.93  &  19.94  &  57346.1  &    9.5  &   \phs$50.7 \pm 2.1$  &  $5.67 \pm 0.93$  &         ...        &  0 \\
DES\,J000224.40$-$605430.0  &    0.60166  & $ -60.90833 $ &  21.67  &  20.73  &  57346.1  &    4.4  &   \phs$78.0 \pm 6.9$  &         ...       &         ...        &  0 \\
DES\,J000225.09$-$603805.0  &    0.60454  & $ -60.63474 $ &  21.22  &  20.68  &  58339.3  &    4.9  &      $-16.5 \pm 3.4$  &  $5.03 \pm 1.29$  &         ...        &  0 \\
DES\,J000225.75$-$605941.8  &    0.60728  & $ -60.99496 $ &  20.53  &  19.76  &  57981.2  &    6.1  &   \phs$40.4 \pm 3.4$  &  $8.26 \pm 1.02$  &         ...        &  0 \\
DES\,J000226.07$-$610125.5  &    0.60861  & $ -61.02374 $ &  21.81  &  20.91  &  58340.3  &    5.9  &  \phs$118.8 \pm 3.0$  &  $3.60 \pm 0.64$  &         ...        &  0 \\
DES\,J000226.82$-$605944.8  &    0.61174  & $ -60.99577 $ &  18.88  &  18.26  &  57981.2  &   17.7  &   \phs$65.2 \pm 1.4$  &  $6.63 \pm 0.42$  &         ...        &  0 \\
DES\,J000228.19$-$604840.7  &    0.61745  & $ -60.81130 $ &  19.84  &  19.40  &  57633.9  &    9.5  &  \phs$219.9 \pm 2.2$  &         ...       &         ...        &  0 \\
DES\,J000228.19$-$604814.3  &    0.61745  & $ -60.80398 $ &  18.88  &  19.03  &  57247.4  &    7.0  &   \phs$12.1 \pm 6.7$  &         ...       &         ...        &  1 \\
                            &    0.61745  & $ -60.80398 $ &  18.88  &  19.03  &  57282.3  &   10.8  &   \phs$10.6 \pm 2.9$  &         ...       &         ...        &  1 \\
                            &    0.61745  & $ -60.80398 $ &  18.88  &  19.03  &  57346.1  &   13.4  &    \phs$8.7 \pm 2.6$  &         ...       &         ...        &  1 \\
                            &    0.61745  & $ -60.80398 $ &  18.88  &  19.03  &  57633.9  &    8.9  &   \phs$10.5 \pm 2.7$  &         ...       &         ...        &  1 \\
                            &    0.61745  & $ -60.80398 $ &  18.88  &  19.03  &  58339.2  &   15.9  &   \phs$24.4 \pm 1.6$  &         ...       &         ...        &  1 \\
                            &    0.61745  & $ -60.80398 $ &  18.88  &  19.03  &  58363.8  &    7.4  &   \phs$14.8 \pm 3.1$  &         ...       &         ...        &  1 \\
DES\,J000229.10$-$604831.4  &    0.62126  & $ -60.80873 $ &  19.01  &  18.36  &  57247.4  &   19.2  &   \phs$73.0 \pm 1.6$  &  $5.68 \pm 0.45$  &         ...        &  0 \\
                            &    0.62126  & $ -60.80873 $ &  19.01  &  18.36  &  57282.3  &   25.2  &   \phs$75.1 \pm 1.4$  &  $6.48 \pm 0.42$  &         ...        &  0 \\
                            &    0.62126  & $ -60.80873 $ &  19.01  &  18.36  &  57346.1  &   30.8  &   \phs$74.0 \pm 1.1$  &  $5.68 \pm 0.37$  &         ...        &  0 \\
                            &    0.62126  & $ -60.80873 $ &  19.01  &  18.36  &  57633.9  &   22.3  &   \phs$72.4 \pm 1.3$  &  $5.79 \pm 0.44$  &         ...        &  0 \\
                            &    0.62126  & $ -60.80873 $ &  19.01  &  18.36  &  58339.2  &   34.3  &   \phs$73.2 \pm 1.1$  &  $5.22 \pm 0.39$  &         ...        &  0 \\
DES\,J000229.39$-$605104.5  &    0.62247  & $ -60.85125 $ &  19.82  &  19.54  &  57633.9  &    5.7  &   \phs$44.8 \pm 8.7$  &         ...       &         ...        &  0 \\
DES\,J000229.59$-$603817.6  &    0.62328  & $ -60.63821 $ &  20.92  &  20.61  &  58339.3  &    4.8  &   \phs$61.2 \pm 8.8$  &         ...       &         ...        &  0 \\
DES\,J000230.25$-$604934.0  &    0.62606  & $ -60.82611 $ &  17.34  &  16.61  &  57247.4  &   59.1  &      $-12.4 \pm 1.2$  &  $6.41 \pm 0.34$  &         ...        &  0 \\
                            &    0.62606  & $ -60.82611 $ &  17.34  &  16.61  &  57282.3  &   72.7  &      $-12.1 \pm 1.2$  &  $6.35 \pm 0.33$  &         ...        &  0 \\
                            &    0.62606  & $ -60.82611 $ &  17.34  &  16.61  &  57346.1  &   83.6  &      $-12.4 \pm 1.0$  &  $6.33 \pm 0.33$  &         ...        &  0 \\
                            &    0.62606  & $ -60.82611 $ &  17.34  &  16.61  &  58339.2  &   90.1  &      $-13.5 \pm 1.0$  &  $5.59 \pm 0.33$  &         ...        &  0 \\
DES\,J000230.83$-$605055.8  &    0.62846  & $ -60.84883 $ &  20.83  &  20.24  &  58339.2  &    8.1  &    \phs$8.6 \pm 1.6$  &         ...       &         ...        &  0 \\
DES\,J000231.53$-$603939.8  &    0.63139  & $ -60.66107 $ &  19.79  &  19.31  &  58339.3  &   15.4  &   \phs$72.1 \pm 1.5$  &  $5.00 \pm 0.59$  &         ...        &  0 \\
DES\,J000232.01$-$604916.8  &    0.63339  & $ -60.82132 $ &  18.84  &  18.47  &  57247.4  &   15.8  &   \phs$17.9 \pm 1.7$  &  $4.43 \pm 0.50$  &         ...        &  0 \\
                            &    0.63339  & $ -60.82132 $ &  18.84  &  18.47  &  57282.3  &   20.3  &   \phs$20.7 \pm 1.4$  &  $3.94 \pm 0.44$  &         ...        &  0 \\
                            &    0.63339  & $ -60.82132 $ &  18.84  &  18.47  &  57346.1  &   25.2  &   \phs$18.8 \pm 1.1$  &  $3.93 \pm 0.37$  &         ...        &  0 \\
                            &    0.63339  & $ -60.82132 $ &  18.84  &  18.47  &  57633.9  &   17.6  &   \phs$17.5 \pm 1.3$  &  $4.38 \pm 0.46$  &         ...        &  0 \\
                            &    0.63339  & $ -60.82132 $ &  18.84  &  18.47  &  58339.2  &   28.5  &   \phs$20.0 \pm 1.1$  &  $3.91 \pm 0.39$  &         ...        &  0 \\
DES\,J000233.86$-$605439.5  &    0.64110  & $ -60.91096 $ &  19.90  &  19.40  &  57247.4  &    7.4  &    \phs$9.8 \pm 2.0$  &  $2.51 \pm 0.83$  &  $-2.28 \pm 0.43$  &  1 \\
                            &    0.64110  & $ -60.91096 $ &  19.90  &  19.40  &  57282.3  &    9.6  &   \phs$11.2 \pm 1.5$  &  $2.33 \pm 0.48$  &  $-2.38 \pm 0.26$  &  1 \\
                            &    0.64110  & $ -60.91096 $ &  19.90  &  19.40  &  57346.1  &   13.0  &    \phs$7.4 \pm 1.4$  &  $3.07 \pm 0.45$  &  $-2.00 \pm 0.22$  &  1 \\
                            &    0.64110  & $ -60.91096 $ &  19.90  &  19.40  &  57633.9  &    8.6  &    \phs$7.3 \pm 1.6$  &  $1.81 \pm 0.35$  &  $-2.67 \pm 0.23$  &  1 \\
                            &    0.64110  & $ -60.91096 $ &  19.90  &  19.40  &  58339.2  &   15.7  &    \phs$9.9 \pm 1.4$  &         ...       &         ...        &  1 \\
DES\,J000234.73$-$605355.8  &    0.64469  & $ -60.89883 $ &  19.42  &  18.85  &  57247.4  &   11.4  &  \phs$124.4 \pm 1.9$  &  $4.72 \pm 0.51$  &         ...        &  0 \\
                            &    0.64469  & $ -60.89883 $ &  19.42  &  18.85  &  57282.3  &   12.6  &  \phs$155.1 \pm 4.4$  &  $6.62 \pm 0.57$  &         ...        &  0 \\
                            &    0.64469  & $ -60.89883 $ &  19.42  &  18.85  &  57346.1  &   16.6  &  \phs$125.8 \pm 1.7$  &         ...       &         ...        &  0 \\
                            &    0.64469  & $ -60.89883 $ &  19.42  &  18.85  &  57633.9  &   13.1  &  \phs$131.7 \pm 2.7$  &         ...       &         ...        &  0 \\
                            &    0.64469  & $ -60.89883 $ &  19.42  &  18.85  &  58339.2  &   21.3  &  \phs$128.3 \pm 1.4$  &         ...       &         ...        &  0 \\
DES\,J000235.08$-$604431.2  &    0.64617  & $ -60.74200 $ &  20.20  &  19.90  &  58339.2  &    9.9  &   \phs$23.9 \pm 1.8$  &  $1.74 \pm 1.30$  &         ...        &  0 \\
DES\,J000236.02$-$605220.5  &    0.65008  & $ -60.87235 $ &  21.04  &  20.51  &  57346.1  &    4.1  &   \phs$87.2 \pm 5.3$  &         ...       &         ...        &  0 \\
                            &    0.65008  & $ -60.87235 $ &  21.04  &  20.51  &  58339.2  &    5.7  &   \phs$95.8 \pm 4.5$  &  $4.44 \pm 0.81$  &         ...        &  0 \\
DES\,J000237.42$-$610020.3  &    0.65592  & $ -61.00565 $ &  20.45  &  19.93  &  58340.3  &   13.6  &  \phs$135.6 \pm 1.5$  &  $4.26 \pm 0.52$  &         ...        &  0 \\
DES\,J000238.21$-$605419.3  &    0.65921  & $ -60.90537 $ &  17.06  &  16.21  &  57633.9  &   88.5  &   \phs$27.6 \pm 1.0$  &         ...       &         ...        &  0 \\
                            &    0.65921  & $ -60.90537 $ &  17.06  &  16.21  &  58339.2  &  103.1  &   \phs$40.4 \pm 1.0$  &  $6.78 \pm 0.33$  &         ...        &  0 \\
DES\,J000239.73$-$604337.2  &    0.66556  & $ -60.72700 $ &  19.45  &  18.49  &  58339.2  &   34.0  &   \phs$63.6 \pm 1.1$  &  $5.69 \pm 0.37$  &         ...        &  0 \\
DES\,J000240.86$-$604527.5  &    0.67025  & $ -60.75763 $ &  21.47  &  20.65  &  58339.2  &    5.9  &   \phs$24.4 \pm 2.7$  &         ...       &         ...        &  0 \\
DES\,J000243.93$-$605518.0  &    0.68306  & $ -60.92166 $ &  20.21  &  19.71  &  57247.4  &    5.1  &  \phs$100.4 \pm 4.0$  &  $5.88 \pm 0.96$  &         ...        &  0 \\
                            &    0.68306  & $ -60.92166 $ &  20.21  &  19.71  &  57282.3  &    7.5  &   \phs$91.4 \pm 5.4$  &  $5.73 \pm 0.86$  &         ...        &  0 \\
                            &    0.68306  & $ -60.92166 $ &  20.21  &  19.71  &  57346.1  &   10.0  &   \phs$97.0 \pm 2.5$  &  $3.48 \pm 0.69$  &         ...        &  0 \\
                            &    0.68306  & $ -60.92166 $ &  20.21  &  19.71  &  57633.9  &    6.8  &   \phs$93.6 \pm 3.0$  &         ...       &         ...        &  0 \\
DES\,J000244.67$-$604819.1  &    0.68615  & $ -60.80531 $ &  20.92  &  20.43  &  57282.3  &    4.1  &   \phs$35.8 \pm 5.8$  &         ...       &         ...        &  0 \\
                            &    0.68615  & $ -60.80531 $ &  20.92  &  20.43  &  58339.2  &    5.4  &   \phs$27.1 \pm 2.4$  &  $3.80 \pm 1.92$  &         ...        &  0 \\
DES\,J000245.85$-$604839.2  &    0.69104  & $ -60.81089 $ &  20.07  &  19.13  &  57247.4  &   11.3  &  \phs$113.8 \pm 2.2$  &  $6.07 \pm 0.68$  &         ...        &  0 \\
                            &    0.69104  & $ -60.81089 $ &  20.07  &  19.13  &  57282.3  &   15.9  &  \phs$115.9 \pm 1.6$  &  $6.69 \pm 0.44$  &         ...        &  0 \\
                            &    0.69104  & $ -60.81089 $ &  20.07  &  19.13  &  57346.1  &   19.2  &  \phs$115.3 \pm 1.5$  &         ...       &         ...        &  0 \\
                            &    0.69104  & $ -60.81089 $ &  20.07  &  19.13  &  57633.9  &   11.5  &  \phs$114.3 \pm 1.5$  &  $6.04 \pm 0.57$  &         ...        &  0 \\
                            &    0.69104  & $ -60.81089 $ &  20.07  &  19.13  &  58339.2  &   22.0  &  \phs$112.4 \pm 1.3$  &  $6.00 \pm 0.43$  &         ...        &  0 \\
DES\,J000246.64$-$604438.4  &    0.69433  & $ -60.74401 $ &  18.30  &  18.00  &  58339.2  &   35.5  &  \phs$115.3 \pm 1.1$  &  $4.47 \pm 0.37$  &         ...        &  0 \\
DES\,J000248.29$-$605445.2  &    0.70122  & $ -60.91254 $ &  19.04  &  18.80  &  57247.4  &   10.9  &  \phs$194.3 \pm 2.1$  &  $1.56 \pm 0.44$  &         ...        &  0 \\
                            &    0.70122  & $ -60.91254 $ &  19.04  &  18.80  &  57282.3  &   11.2  &  \phs$198.2 \pm 1.6$  &  $1.91 \pm 0.48$  &         ...        &  0 \\
                            &    0.70122  & $ -60.91254 $ &  19.04  &  18.80  &  57346.1  &   14.4  &  \phs$201.1 \pm 1.5$  &         ...       &         ...        &  0 \\
                            &    0.70122  & $ -60.91254 $ &  19.04  &  18.80  &  57633.9  &   12.9  &  \phs$198.1 \pm 1.8$  &  $1.87 \pm 0.44$  &         ...        &  0 \\
DES\,J000251.06$-$610131.1  &    0.71274  & $ -61.02531 $ &  18.08  &  17.52  &  58340.3  &   65.1  &      $-55.0 \pm 1.0$  &  $5.41 \pm 0.33$  &         ...        &  0 \\
DES\,J000251.92$-$604820.8  &    0.71632  & $ -60.80577 $ &  19.57  &  19.08  &  57247.4  &   10.2  &   \phs$11.6 \pm 1.6$  &  $2.98 \pm 1.16$  &  $-2.12 \pm 0.56$  &  1 \\
                            &    0.71632  & $ -60.80577 $ &  19.57  &  19.08  &  57282.3  &   14.7  &   \phs$12.2 \pm 1.5$  &  $1.92 \pm 0.50$  &  $-2.67 \pm 0.30$  &  1 \\
                            &    0.71632  & $ -60.80577 $ &  19.57  &  19.08  &  57346.1  &   17.9  &    \phs$8.4 \pm 1.2$  &  $1.71 \pm 0.37$  &  $-2.79 \pm 0.25$  &  1 \\
                            &    0.71632  & $ -60.80577 $ &  19.57  &  19.08  &  57633.9  &   12.2  &    \phs$7.6 \pm 1.6$  &  $1.71 \pm 0.37$  &  $-2.80 \pm 0.25$  &  1 \\
                            &    0.71632  & $ -60.80577 $ &  19.57  &  19.08  &  58339.2  &   18.2  &    \phs$8.5 \pm 1.2$  &  $1.98 \pm 0.37$  &  $-2.64 \pm 0.22$  &  1 \\
                            &    0.71632  & $ -60.80577 $ &  19.57  &  19.08  &  58363.8  &   10.8  &   \phs$10.5 \pm 1.7$  &  $2.13 \pm 0.45$  &  $-2.55 \pm 0.25$  &  1 \\
DES\,J000252.35$-$604407.2  &    0.71812  & $ -60.73533 $ &  20.85  &  20.25  &  58339.2  &    6.9  &  \phs$162.0 \pm 2.8$  &  $4.89 \pm 0.70$  &         ...        &  0 \\
DES\,J000252.68$-$604750.4  &    0.71950  & $ -60.79733 $ &  20.69  &  20.03  &  58339.2  &    9.2  &  \phs$104.1 \pm 2.0$  &  $5.03 \pm 0.73$  &         ...        &  0 \\
DES\,J000252.79$-$605346.8  &    0.71997  & $ -60.89634 $ &  20.62  &  20.11  &  57282.3  &    5.2  &       $-4.1 \pm 2.8$  &  $3.02 \pm 0.82$  &         ...        &  0 \\
                            &    0.71997  & $ -60.89634 $ &  20.62  &  20.11  &  57346.1  &    6.8  &       $-5.2 \pm 2.6$  &  $4.36 \pm 0.70$  &         ...        &  0 \\
                            &    0.71997  & $ -60.89634 $ &  20.62  &  20.11  &  57633.9  &    5.0  &       $-7.5 \pm 6.3$  &         ...       &         ...        &  0 \\
                            &    0.71997  & $ -60.89634 $ &  20.62  &  20.11  &  58339.2  &    7.4  &       $-4.9 \pm 2.3$  &  $4.86 \pm 0.80$  &         ...        &  0 \\
DES\,J000253.10$-$610013.5  &    0.72126  & $ -61.00374 $ &  20.13  &  19.88  &  58340.3  &   12.1  &  \phs$226.0 \pm 1.7$  &  $1.80 \pm 0.46$  &         ...        &  0 \\
DES\,J000254.13$-$604625.3  &    0.72555  & $ -60.77370 $ &  20.44  &  20.07  &  58339.2  &    7.4  &  \phs$272.1 \pm 2.5$  &  $2.62 \pm 0.72$  &         ...        &  0 \\
DES\,J000254.31$-$603806.0  &    0.72628  & $ -60.63500 $ &  20.21  &  19.93  &  58339.3  &    8.2  &  \phs$133.9 \pm 1.8$  &  $2.66 \pm 0.60$  &         ...        &  0 \\
DES\,J000257.02$-$605140.0  &    0.73757  & $ -60.86111 $ &  20.27  &  19.80  &  57247.4  &    5.1  &   \phs$14.7 \pm 2.8$  &  $2.67 \pm 0.57$  &  $-2.12 \pm 0.30$  &  1 \\
                            &    0.73757  & $ -60.86111 $ &  20.27  &  19.80  &  57282.3  &    8.2  &   \phs$15.0 \pm 2.0$  &  $2.05 \pm 0.40$  &  $-2.45 \pm 0.24$  &  1 \\
                            &    0.73757  & $ -60.86111 $ &  20.27  &  19.80  &  57346.1  &   10.3  &   \phs$14.9 \pm 2.1$  &  $2.97 \pm 0.52$  &  $-1.97 \pm 0.26$  &  1 \\
                            &    0.73757  & $ -60.86111 $ &  20.27  &  19.80  &  57633.9  &    6.1  &   \phs$20.5 \pm 2.1$  &  $1.71 \pm 0.55$  &  $-2.66 \pm 0.36$  &  1 \\
                            &    0.73757  & $ -60.86111 $ &  20.27  &  19.80  &  58339.2  &   10.9  &   \phs$15.2 \pm 1.5$  &  $3.00 \pm 0.60$  &  $-1.95 \pm 0.30$  &  1 \\
                            &    0.73757  & $ -60.86111 $ &  20.27  &  19.80  &  58363.8  &    5.1  &   \phs$18.6 \pm 3.0$  &  $2.75 \pm 0.96$  &  $-2.08 \pm 0.49$  &  1 \\
DES\,J000257.12$-$604330.2  &    0.73798  & $ -60.72506 $ &  20.62  &  20.37  &  58339.2  &    4.6  &  \phs$298.0 \pm 2.9$  &         ...       &         ...        &  0 \\
DES\,J000300.17$-$604040.9  &    0.75069  & $ -60.67802 $ &  20.31  &  19.47  &  58339.2  &   13.5  &       $-4.3 \pm 1.6$  &  $4.28 \pm 0.56$  &         ...        &  0 \\
                            &    0.75069  & $ -60.67802 $ &  20.31  &  19.47  &  58339.3  &   11.9  &       $-1.5 \pm 1.5$  &  $5.31 \pm 0.64$  &         ...        &  0 \\
DES\,J000300.40$-$605144.8  &    0.75167  & $ -60.86244 $ &  20.45  &  20.16  &  57633.9  &    4.8  &     $-205.4 \pm 5.2$  &         ...       &         ...        &  0 \\
DES\,J000301.29$-$610447.0  &    0.75539  & $ -61.07972 $ &  18.94  &  18.01  &  58340.3  &   52.0  &    \phs$4.5 \pm 1.0$  &  $6.13 \pm 0.34$  &         ...        &  0 \\
DES\,J000302.47$-$610611.2  &    0.76029  & $ -61.10312 $ &  20.80  &  20.13  &  58340.3  &    8.9  &   \phs$61.4 \pm 2.2$  &  $5.89 \pm 0.79$  &         ...        &  0 \\
DES\,J000302.63$-$604730.5  &    0.76096  & $ -60.79181 $ &  20.78  &  19.92  &  58339.2  &   10.9  &   \phs$52.5 \pm 1.6$  &  $7.22 \pm 0.58$  &         ...        &  0 \\
DES\,J000303.55$-$605025.3  &    0.76480  & $ -60.84036 $ &  18.79  &  18.88  &  57247.4  &    8.6  &   \phs$22.1 \pm 2.7$  &         ...       &         ...        &  1 \\
                            &    0.76480  & $ -60.84036 $ &  18.79  &  18.88  &  57282.3  &    9.2  &   \phs$18.5 \pm 2.0$  &         ...       &         ...        &  1 \\
                            &    0.76480  & $ -60.84036 $ &  18.79  &  18.88  &  57346.1  &   10.0  &   \phs$19.9 \pm 3.5$  &         ...       &         ...        &  1 \\
                            &    0.76480  & $ -60.84036 $ &  18.79  &  18.88  &  57633.9  &    7.7  &   \phs$11.7 \pm 2.3$  &         ...       &         ...        &  1 \\
                            &    0.76480  & $ -60.84036 $ &  18.79  &  18.88  &  58339.2  &   15.3  &   \phs$20.5 \pm 1.7$  &         ...       &         ...        &  1 \\
                            &    0.76480  & $ -60.84036 $ &  18.79  &  18.88  &  58363.8  &    9.1  &   \phs$16.9 \pm 2.6$  &         ...       &         ...        &  1 \\
DES\,J000304.42$-$603742.9  &    0.76843  & $ -60.62858 $ &  21.04  &  20.47  &  58339.3  &    5.2  &   \phs$52.5 \pm 3.9$  &  $6.38 \pm 1.17$  &         ...        &  0 \\
DES\,J000305.83$-$611143.7  &    0.77431  & $ -61.19548 $ &  18.80  &  18.22  &  58340.1  &   15.7  &   \phs$17.7 \pm 1.1$  &  $2.57 \pm 0.40$  &  $-2.49 \pm 0.20$  &  1 \\
DES\,J000307.48$-$604800.5  &    0.78119  & $ -60.80013 $ &  19.15  &  18.33  &  57247.4  &   16.0  &    \phs$7.0 \pm 1.7$  &         ...       &         ...        &  0 \\
                            &    0.78119  & $ -60.80013 $ &  19.15  &  18.33  &  57282.3  &   27.2  &    \phs$2.4 \pm 1.3$  &         ...       &         ...        &  0 \\
                            &    0.78119  & $ -60.80013 $ &  19.15  &  18.33  &  57346.1  &   32.0  &    \phs$3.7 \pm 1.1$  &  $6.05 \pm 0.37$  &         ...        &  0 \\
                            &    0.78119  & $ -60.80013 $ &  19.15  &  18.33  &  58339.2  &   30.9  &    \phs$5.4 \pm 1.1$  &  $6.25 \pm 0.37$  &         ...        &  0 \\
DES\,J000308.38$-$610123.0  &    0.78492  & $ -61.02305 $ &  20.57  &  19.74  &  58340.3  &   16.3  &   \phs$67.4 \pm 4.4$  &  $7.24 \pm 0.90$  &         ...        &  0 \\
DES\,J000308.56$-$604725.3  &    0.78568  & $ -60.79037 $ &  18.67  &  18.37  &  58339.2  &   26.2  &  \phs$189.4 \pm 1.1$  &  $2.22 \pm 0.41$  &         ...        &  0 \\
DES\,J000311.46$-$604451.5  &    0.79776  & $ -60.74764 $ &  18.11  &  17.35  &  57247.4  &   41.7  &   \phs$14.6 \pm 1.2$  &  $5.18 \pm 0.35$  &         ...        &  0 \\
                            &    0.79776  & $ -60.74764 $ &  18.11  &  17.35  &  57282.3  &   52.4  &   \phs$14.6 \pm 1.2$  &  $5.23 \pm 0.34$  &         ...        &  0 \\
                            &    0.79776  & $ -60.74764 $ &  18.11  &  17.35  &  57346.1  &   60.2  &   \phs$14.9 \pm 1.0$  &  $5.32 \pm 0.33$  &         ...        &  0 \\
DES\,J000312.54$-$605608.4  &    0.80225  & $ -60.93566 $ &  18.99  &  18.66  &  57633.9  &   14.3  &  \phs$155.1 \pm 1.4$  &  $2.55 \pm 0.57$  &         ...        &  0 \\
DES\,J000313.03$-$604332.5  &    0.80430  & $ -60.72569 $ &  19.11  &  18.89  &  57247.4  &   10.8  &   \phs$35.8 \pm 1.9$  &  $1.50 \pm 0.54$  &         ...        &  0 \\
                            &    0.80430  & $ -60.72569 $ &  19.11  &  18.89  &  57282.3  &   14.3  &   \phs$37.9 \pm 1.8$  &  $2.41 \pm 0.72$  &         ...        &  0 \\
                            &    0.80430  & $ -60.72569 $ &  19.11  &  18.89  &  57346.1  &   17.5  &   \phs$38.4 \pm 1.3$  &  $1.65 \pm 0.37$  &         ...        &  0 \\
DES\,J000313.56$-$610318.4  &    0.80648  & $ -61.05511 $ &  20.75  &  20.28  &  58340.3  &    7.7  &      $-10.4 \pm 2.0$  &  $2.23 \pm 0.80$  &         ...        &  0 \\
DES\,J000314.87$-$603722.3  &    0.81198  & $ -60.62286 $ &  20.42  &  19.96  &  58339.3  &    9.2  &  \phs$117.1 \pm 1.9$  &  $2.73 \pm 0.44$  &         ...        &  0 \\
DES\,J000315.49$-$604456.1  &    0.81454  & $ -60.74891 $ &  20.01  &  19.79  &  57247.4  &    5.1  &      $-23.7 \pm 2.8$  &         ...       &         ...        &  0 \\
                            &    0.81454  & $ -60.74891 $ &  20.01  &  19.79  &  57282.3  &    6.8  &      $-17.6 \pm 2.9$  &  $2.12 \pm 0.76$  &         ...        &  0 \\
                            &    0.81454  & $ -60.74891 $ &  20.01  &  19.79  &  57346.1  &    7.7  &      $-16.7 \pm 2.0$  &  $1.98 \pm 0.51$  &         ...        &  0 \\
DES\,J000317.46$-$604733.8  &    0.82274  & $ -60.79271 $ &  20.84  &  20.40  &  57282.3  &    4.2  &  \phs$113.6 \pm 8.4$  &         ...       &         ...        &  0 \\
                            &    0.82274  & $ -60.79271 $ &  20.84  &  20.40  &  57346.1  &    5.8  &  \phs$106.0 \pm 7.7$  &  $4.41 \pm 0.55$  &         ...        &  0 \\
DES\,J000317.78$-$604652.2  &    0.82407  & $ -60.78116 $ &  19.71  &  19.23  &  57247.4  &    7.9  &   \phs$38.8 \pm 2.7$  &         ...       &         ...        &  0 \\
                            &    0.82407  & $ -60.78116 $ &  19.71  &  19.23  &  57282.3  &   11.9  &   \phs$31.8 \pm 2.0$  &         ...       &         ...        &  0 \\
                            &    0.82407  & $ -60.78116 $ &  19.71  &  19.23  &  57346.1  &   14.3  &   \phs$32.3 \pm 1.4$  &  $5.90 \pm 0.64$  &         ...        &  0 \\
DES\,J000321.45$-$604246.1  &    0.83939  & $ -60.71282 $ &  20.02  &  19.66  &  57247.4  &    5.3  &  \phs$215.7 \pm 3.8$  &  $1.60 \pm 0.58$  &         ...        &  0 \\
                            &    0.83939  & $ -60.71282 $ &  20.02  &  19.66  &  57282.3  &    7.2  &  \phs$223.2 \pm 2.2$  &         ...       &         ...        &  0 \\
                            &    0.83939  & $ -60.71282 $ &  20.02  &  19.66  &  57346.1  &    9.4  &  \phs$219.8 \pm 1.8$  &         ...       &         ...        &  0 \\
                            &    0.83939  & $ -60.71282 $ &  20.02  &  19.66  &  58339.2  &    7.5  &  \phs$222.2 \pm 2.6$  &         ...       &         ...        &  0 \\
DES\,J000324.55$-$604319.0  &    0.85231  & $ -60.72195 $ &  18.82  &  18.54  &  57247.4  &   14.7  &  \phs$126.0 \pm 2.6$  &  $0.63 \pm 0.38$  &         ...        &  0 \\
                            &    0.85231  & $ -60.72195 $ &  18.82  &  18.54  &  57282.3  &   18.6  &  \phs$127.4 \pm 3.2$  &  $0.44 \pm 0.32$  &         ...        &  0 \\
                            &    0.85231  & $ -60.72195 $ &  18.82  &  18.54  &  57346.1  &   22.2  &  \phs$130.7 \pm 1.4$  &  $1.30 \pm 0.35$  &         ...        &  0 \\
DES\,J000326.98$-$604234.8  &    0.86240  & $ -60.70968 $ &  20.91  &  20.46  &  57282.3  &    4.1  &   \phs$22.3 \pm 2.8$  &  $3.05 \pm 0.51$  &  $-1.79 \pm 0.26$  &  1 \\
                            &    0.86240  & $ -60.70968 $ &  20.91  &  20.46  &  57346.1  &    5.4  &   \phs$17.5 \pm 3.0$  &  $1.87 \pm 0.67$  &  $-2.43 \pm 0.42$  &  1 \\
DES\,J000329.11$-$604847.0  &    0.87129  & $ -60.81306 $ &  19.70  &  18.93  &  57247.4  &   12.4  &   \phs$56.8 \pm 1.8$  &  $6.24 \pm 0.80$  &         ...        &  0 \\
                            &    0.87129  & $ -60.81306 $ &  19.70  &  18.93  &  57282.3  &   15.4  &   \phs$57.6 \pm 1.6$  &  $7.12 \pm 0.53$  &         ...        &  0 \\
                            &    0.87129  & $ -60.81306 $ &  19.70  &  18.93  &  57346.1  &   18.8  &   \phs$55.7 \pm 1.3$  &  $6.23 \pm 0.44$  &         ...        &  0 \\
DES\,J000331.90$-$604623.1  &    0.88292  & $ -60.77307 $ &  19.33  &  18.46  &  57247.4  &   17.9  &   \phs$54.3 \pm 1.5$  &  $6.64 \pm 0.41$  &         ...        &  0 \\
                            &    0.88292  & $ -60.77307 $ &  19.33  &  18.46  &  57282.3  &   22.4  &   \phs$55.0 \pm 1.4$  &  $6.38 \pm 0.42$  &         ...        &  0 \\
                            &    0.88292  & $ -60.77307 $ &  19.33  &  18.46  &  57346.1  &   27.4  &   \phs$57.2 \pm 1.1$  &  $5.91 \pm 0.40$  &         ...        &  0 \\
DES\,J000335.45$-$604829.5  &    0.89771  & $ -60.80821 $ &  20.25  &  19.76  &  57247.4  &    5.7  &      $-43.4 \pm 6.2$  &  $3.30 \pm 0.69$  &         ...        &  0 \\
                            &    0.89771  & $ -60.80821 $ &  20.25  &  19.76  &  57282.3  &    6.5  &      $-33.8 \pm 2.6$  &         ...       &         ...        &  0 \\
                            &    0.89771  & $ -60.80821 $ &  20.25  &  19.76  &  57346.1  &    8.9  &      $-34.8 \pm 2.0$  &  $4.49 \pm 0.71$  &         ...        &  0 \\
DES\,J000344.06$-$604804.7  &    0.93358  & $ -60.80130 $ &  18.84  &  19.00  &  57247.4  &    6.3  &   \phs$21.4 \pm 3.7$  &         ...       &         ...        &  1 \\
                            &    0.93358  & $ -60.80130 $ &  18.84  &  19.00  &  57282.3  &    8.4  &   \phs$20.7 \pm 2.7$  &         ...       &         ...        &  1 \\
                            &    0.93358  & $ -60.80130 $ &  18.84  &  19.00  &  57346.1  &   11.5  &   \phs$21.1 \pm 1.9$  &         ...       &         ...        &  1 \\
DES\,J000352.62$-$604702.5  &    0.96924  & $ -60.78402 $ &  19.79  &  19.48  &  57247.4  &    5.9  &  \phs$143.3 \pm 2.6$  &  $3.45 \pm 0.44$  &         ...        &  0 \\
                            &    0.96924  & $ -60.78402 $ &  19.79  &  19.48  &  57282.3  &    6.8  &  \phs$144.6 \pm 2.2$  &  $4.11 \pm 0.62$  &         ...        &  0 \\
                            &    0.96924  & $ -60.78402 $ &  19.79  &  19.48  &  57346.1  &    9.2  &  \phs$146.0 \pm 1.8$  &  $4.09 \pm 0.66$  &         ...        &  0 \\
DES\,J000415.35$-$605008.7  &    1.06395  & $ -60.83574 $ &  19.64  &  19.02  &  57982.1  &   11.4  &  \phs$117.1 \pm 2.1$  &  $4.55 \pm 0.51$  &         ...        &  0 \\
DES\,J000423.90$-$604805.4  &    1.09957  & $ -60.80151 $ &  18.01  &  17.46  &  57982.1  &   31.0  &   \phs$88.5 \pm 1.1$  &  $5.13 \pm 0.37$  &         ...        &  0 \\
DES\,J000424.12$-$605043.5  &    1.10050  & $ -60.84542 $ &  21.21  &  20.23  &  57982.1  &    4.5  &  \phs$110.8 \pm 2.7$  &         ...       &         ...        &  0 \\
DES\,J000426.13$-$604911.2  &    1.10889  & $ -60.81978 $ &  20.02  &  19.59  &  57982.1  &    6.5  &  \phs$177.6 \pm 2.3$  &  $3.28 \pm 0.65$  &         ...        &  0 \\
DES\,J000429.02$-$604242.2  &    1.12092  & $ -60.71172 $ &  19.90  &  19.31  &  57982.1  &    9.3  &   \phs$14.6 \pm 1.7$  &  $5.43 \pm 0.57$  &         ...        &  0 \\
DES\,J000431.02$-$604323.7  &    1.12926  & $ -60.72325 $ &  20.83  &  19.87  &  57982.1  &    6.8  &   \phs$18.2 \pm 1.7$  &  $5.89 \pm 0.61$  &         ...        &  0 \\
DES\,J000433.12$-$604733.9  &    1.13802  & $ -60.79274 $ &  19.02  &  18.59  &  57982.1  &   14.2  &  \phs$106.1 \pm 1.6$  &         ...       &         ...        &  0 \\
DES\,J000436.03$-$605117.1  &    1.15012  & $ -60.85474 $ &  18.89  &  18.78  &  57982.1  &   11.2  &  \phs$109.6 \pm 2.2$  &         ...       &         ...        &  0 \\
DES\,J000437.90$-$604453.8  &    1.15793  & $ -60.74829 $ &  20.25  &  19.89  &  57982.1  &    5.5  &  \phs$348.9 \pm 3.4$  &         ...       &         ...        &  0 \\
DES\,J000441.56$-$605213.3  &    1.17318  & $ -60.87037 $ &  20.83  &  20.24  &  57982.1  &    4.1  &   \phs$37.6 \pm 3.6$  &         ...       &         ...        &  0 \\
DES\,J000443.33$-$605207.8  &    1.18052  & $ -60.86884 $ &  19.77  &  19.35  &  57982.1  &    8.1  &  \phs$155.1 \pm 1.7$  &  $1.97 \pm 0.52$  &         ...        &  0 \\
DES\,J000445.28$-$604743.2  &    1.18865  & $ -60.79533 $ &  20.34  &  20.00  &  57982.1  &    4.3  &      $-28.7 \pm 6.3$  &         ...       &         ...        &  0 \\
DES\,J000451.75$-$604906.3  &    1.21564  & $ -60.81842 $ &  19.74  &  19.50  &  57982.1  &    6.5  &      $-45.4 \pm 2.7$  &         ...       &         ...        &  0 \\
DES\,J000451.87$-$604103.8  &    1.21613  & $ -60.68440 $ &  19.49  &  18.94  &  57982.1  &    8.5  &  \phs$107.0 \pm 2.2$  &         ...       &         ...        &  0 \\
DES\,J000453.28$-$603938.5  &    1.22199  & $ -60.66068 $ &  19.25  &  18.53  &  57982.1  &   11.6  &   \phs$17.8 \pm 1.5$  &  $5.48 \pm 0.61$  &         ...        &  0 \\
DES\,J000456.16$-$604945.8  &    1.23401  & $ -60.82938 $ &  19.42  &  19.17  &  57982.1  &    8.2  &  \phs$254.6 \pm 2.2$  &         ...       &         ...        &  0 \\
DES\,J000456.81$-$604842.1  &    1.23671  & $ -60.81170 $ &  19.16  &  18.68  &  57982.1  &   12.9  &   \phs$45.0 \pm 1.3$  &  $5.09 \pm 0.50$  &         ...        &  0 \\
DES\,J000459.73$-$605147.6  &    1.24887  & $ -60.86322 $ &  19.77  &  19.28  &  57982.1  &    8.6  &  \phs$188.2 \pm 2.8$  &  $4.99 \pm 0.75$  &         ...        &  0 \\
DES\,J000501.31$-$604504.2  &    1.25544  & $ -60.75118 $ &  19.79  &  18.99  &  57982.1  &   11.8  &  \phs$155.2 \pm 1.6$  &         ...       &         ...        &  0 \\
DES\,J000501.50$-$604830.5  &    1.25625  & $ -60.80847 $ &  18.33  &  18.11  &  57982.1  &   17.0  &  \phs$282.4 \pm 1.4$  &  $4.14 \pm 0.40$  &         ...        &  0 \\
DES\,J000504.68$-$604648.9  &    1.26951  & $ -60.78025 $ &  18.20  &  17.49  &  57982.1  &   27.2  &    \phs$6.6 \pm 1.1$  &  $6.02 \pm 0.40$  &         ...        &  0 \\
DES\,J000508.41$-$604356.2  &    1.28504  & $ -60.73228 $ &  19.63  &  19.15  &  57982.1  &    6.2  &      $-11.6 \pm 3.7$  &  $4.35 \pm 1.14$  &         ...        &  0 \\
DES\,J000511.50$-$604441.2  &    1.29793  & $ -60.74478 $ &  20.18  &  19.52  &  57982.1  &    4.6  &  \phs$122.9 \pm 7.1$  &  $5.93 \pm 1.52$  &         ...        &  0 \\
DES\,J000516.62$-$603946.7  &    1.31927  & $ -60.66296 $ &  18.98  &  18.17  &  57982.1  &   11.8  &  \phs$149.5 \pm 1.9$  &  $5.46 \pm 0.61$  &         ...        &  0 \\
DES\,J233632.23$-$631542.1  &  354.13427  & $ -63.26169 $ &  21.13  &  20.60  &  57568.7  &    4.9  &  \phs$184.4 \pm 4.9$  &         ...       &         ...        &  0 \\
DES\,J233646.49$-$632018.7  &  354.19369  & $ -63.33853 $ &  16.70  &  16.02  &  57283.3  &   57.6  &      $-18.8 \pm 1.2$  &  $5.76 \pm 0.34$  &         ...        &  0 \\
                            &  354.19369  & $ -63.33853 $ &  16.70  &  16.02  &  57312.2  &   86.3  &      $-16.1 \pm 1.2$  &         ...       &         ...        &  0 \\
                            &  354.19369  & $ -63.33853 $ &  16.70  &  16.02  &  57568.7  &  155.1  &      $-17.1 \pm 1.0$  &  $6.05 \pm 0.32$  &         ...        &  0 \\
DES\,J233649.07$-$631738.1  &  354.20444  & $ -63.29392 $ &  19.23  &  18.57  &  57283.3  &   11.8  &      $-16.8 \pm 1.8$  &         ...       &         ...        &  0 \\
                            &  354.20444  & $ -63.29392 $ &  19.23  &  18.57  &  57312.2  &   18.5  &      $-15.6 \pm 1.5$  &         ...       &         ...        &  0 \\
                            &  354.20444  & $ -63.29392 $ &  19.23  &  18.57  &  57568.7  &   31.9  &      $-14.9 \pm 1.1$  &  $5.46 \pm 0.44$  &         ...        &  0 \\
DES\,J233652.04$-$631849.2  &  354.21685  & $ -63.31367 $ &  19.87  &  19.60  &  57312.2  &    6.3  &      $-18.9 \pm 2.3$  &  $4.04 \pm 0.78$  &         ...        &  0 \\
                            &  354.21685  & $ -63.31367 $ &  19.87  &  19.60  &  57568.7  &   12.8  &      $-16.2 \pm 1.6$  &  $2.68 \pm 0.68$  &         ...        &  0 \\
DES\,J233653.85$-$631703.9  &  354.22436  & $ -63.28442 $ &  21.06  &  20.62  &  57568.7  &    5.0  &      $-36.8 \pm 3.5$  &         ...       &         ...        &  1 \\
DES\,J233655.57$-$631830.3  &  354.23154  & $ -63.30841 $ &  20.92  &  20.46  &  57568.7  &    6.3  &   \phs$50.9 \pm 2.4$  &  $2.55 \pm 0.70$  &         ...        &  0 \\
DES\,J233707.00$-$631807.1  &  354.27915  & $ -63.30198 $ &  20.60  &  20.14  &  57312.2  &    4.3  &    \phs$4.5 \pm 6.0$  &  $3.68 \pm 1.85$  &         ...        &  0 \\
                            &  354.27915  & $ -63.30198 $ &  20.60  &  20.14  &  57568.7  &    7.8  &       $-2.7 \pm 3.3$  &         ...       &         ...        &  0 \\
DES\,J233712.54$-$631902.1  &  354.30225  & $ -63.31726 $ &  20.90  &  20.61  &  57568.7  &    5.3  &  \phs$184.1 \pm 9.6$  &  $3.53 \pm 0.68$  &         ...        &  0 \\
DES\,J233717.28$-$631536.5  &  354.32199  & $ -63.26015 $ &  20.60  &  20.10  &  57312.2  &    5.0  &      $-35.9 \pm 4.1$  &         ...       &         ...        &  1 \\
                            &  354.32199  & $ -63.26015 $ &  20.60  &  20.10  &  57568.7  &    9.8  &      $-33.9 \pm 1.5$  &  $1.77 \pm 0.44$  &  $-2.62 \pm 0.29$  &  1 \\
DES\,J233722.59$-$631749.6  &  354.34412  & $ -63.29712 $ &  21.13  &  20.62  &  57568.7  &    6.2  &   \phs$40.8 \pm 2.3$  &  $4.69 \pm 0.60$  &         ...        &  0 \\
DES\,J233732.50$-$631428.5  &  354.38543  & $ -63.24125 $ &  20.73  &  20.48  &  57568.7  &    6.2  &  \phs$223.1 \pm 5.4$  &         ...       &         ...        &  0 \\
DES\,J233737.97$-$631159.5  &  354.40820  & $ -63.19987 $ &  20.43  &  19.94  &  57283.3  &    4.2  &  \phs$127.1 \pm 8.6$  &  $5.23 \pm 0.96$  &         ...        &  0 \\
                            &  354.40820  & $ -63.19987 $ &  20.43  &  19.94  &  57312.2  &    6.7  &  \phs$122.6 \pm 3.6$  &  $3.47 \pm 0.76$  &         ...        &  0 \\
                            &  354.40820  & $ -63.19987 $ &  20.43  &  19.94  &  57568.7  &   13.0  &  \phs$128.8 \pm 1.9$  &  $5.06 \pm 0.53$  &         ...        &  0 \\
DES\,J233744.80$-$631750.5  &  354.43665  & $ -63.29735 $ &  19.22  &  18.74  &  57283.3  &   10.5  &   \phs$15.9 \pm 1.8$  &  $4.88 \pm 0.61$  &         ...        &  0 \\
                            &  354.43665  & $ -63.29735 $ &  19.22  &  18.74  &  57312.2  &   15.5  &   \phs$12.3 \pm 1.5$  &  $5.57 \pm 0.50$  &         ...        &  0 \\
                            &  354.43665  & $ -63.29735 $ &  19.22  &  18.74  &  57568.7  &   22.1  &   \phs$13.7 \pm 1.2$  &  $5.77 \pm 0.45$  &         ...        &  0 \\
DES\,J233746.30$-$631329.1  &  354.44292  & $ -63.22475 $ &  19.42  &  18.85  &  57283.3  &   11.0  &      $-37.1 \pm 1.6$  &  $3.16 \pm 0.74$  &  $-2.15 \pm 0.35$  &  1 \\
                            &  354.44292  & $ -63.22475 $ &  19.42  &  18.85  &  57312.2  &   16.7  &      $-37.4 \pm 1.4$  &  $3.67 \pm 0.52$  &  $-1.92 \pm 0.24$  &  1 \\
                            &  354.44292  & $ -63.22475 $ &  19.42  &  18.85  &  57568.7  &   31.3  &      $-37.7 \pm 1.1$  &  $3.76 \pm 0.38$  &  $-1.87 \pm 0.18$  &  1 \\
DES\,J233746.86$-$631441.6  &  354.44523  & $ -63.24490 $ &  20.77  &  19.94  &  57312.2  &    5.6  &      $-54.2 \pm 2.2$  &  $4.82 \pm 1.18$  &         ...        &  0 \\
                            &  354.44523  & $ -63.24490 $ &  20.77  &  19.94  &  57568.7  &   13.0  &      $-58.1 \pm 1.7$  &  $5.33 \pm 0.55$  &         ...        &  0 \\
DES\,J233747.80$-$631228.6  &  354.44915  & $ -63.20794 $ &  20.09  &  19.52  &  57283.3  &    6.6  &  \phs$107.7 \pm 3.4$  &  $4.54 \pm 1.03$  &         ...        &  0 \\
                            &  354.44915  & $ -63.20794 $ &  20.09  &  19.52  &  57312.2  &    8.9  &  \phs$113.4 \pm 2.1$  &         ...       &         ...        &  0 \\
                            &  354.44915  & $ -63.20794 $ &  20.09  &  19.52  &  57568.7  &   18.0  &  \phs$110.4 \pm 1.4$  &  $4.70 \pm 0.52$  &         ...        &  0 \\
DES\,J233750.05$-$631137.9  &  354.45855  & $ -63.19386 $ &  21.17  &  20.57  &  57568.7  &    8.0  &  \phs$332.6 \pm 2.2$  &  $4.66 \pm 0.61$  &         ...        &  0 \\
DES\,J233755.82$-$631322.1  &  354.48259  & $ -63.22281 $ &  20.91  &  20.63  &  57568.7  &    5.6  &  \phs$223.7 \pm 6.2$  &         ...       &         ...        &  0 \\
DES\,J233759.93$-$631136.7  &  354.49970  & $ -63.19351 $ &  18.31  &  17.65  &  57283.3  &   25.4  &   \phs$50.2 \pm 1.4$  &  $6.11 \pm 0.40$  &         ...        &  0 \\
                            &  354.49970  & $ -63.19351 $ &  18.31  &  17.65  &  57312.2  &   38.6  &   \phs$48.6 \pm 1.3$  &  $5.62 \pm 0.36$  &         ...        &  0 \\
                            &  354.49970  & $ -63.19351 $ &  18.31  &  17.65  &  57568.7  &   72.4  &   \phs$49.0 \pm 1.0$  &  $5.88 \pm 0.33$  &         ...        &  0 \\
DES\,J233760.00$-$631442.2  &  354.50000  & $ -63.24505 $ &  19.15  &  18.69  &  57283.3  &   11.0  &   \phs$41.2 \pm 2.2$  &         ...       &         ...        &  0 \\
                            &  354.50000  & $ -63.24505 $ &  19.15  &  18.69  &  57312.2  &   16.7  &   \phs$42.9 \pm 1.8$  &  $5.65 \pm 0.49$  &         ...        &  0 \\
                            &  354.50000  & $ -63.24505 $ &  19.15  &  18.69  &  57568.7  &   30.5  &   \phs$40.9 \pm 1.1$  &  $5.97 \pm 0.38$  &         ...        &  0 \\
DES\,J233813.91$-$631537.8  &  354.55794  & $ -63.26051 $ &  19.86  &  18.88  &  57283.3  &   11.7  &   \phs$73.7 \pm 2.2$  &  $5.68 \pm 0.59$  &         ...        &  0 \\
                            &  354.55794  & $ -63.26051 $ &  19.86  &  18.88  &  57312.2  &   17.6  &   \phs$74.6 \pm 1.5$  &  $5.10 \pm 0.47$  &         ...        &  0 \\
                            &  354.55794  & $ -63.26051 $ &  19.86  &  18.88  &  57568.7  &   23.8  &   \phs$73.9 \pm 1.2$  &  $5.56 \pm 0.42$  &         ...        &  0 \\
DES\,J233814.15$-$631047.4  &  354.55897  & $ -63.17983 $ &  20.62  &  19.63  &  57283.3  &    6.8  &   \phs$97.6 \pm 5.4$  &         ...       &         ...        &  0 \\
                            &  354.55897  & $ -63.17983 $ &  20.62  &  19.63  &  57312.2  &    9.3  &  \phs$125.2 \pm 5.1$  &  $4.94 \pm 0.70$  &         ...        &  0 \\
                            &  354.55897  & $ -63.17983 $ &  20.62  &  19.63  &  57568.7  &   20.1  &  \phs$143.4 \pm 3.7$  &  $5.81 \pm 0.61$  &         ...        &  0 \\
DES\,J233814.40$-$631117.3  &  354.56001  & $ -63.18814 $ &  21.19  &  20.63  &  57568.7  &    6.2  &  \phs$286.1 \pm 2.7$  &         ...       &         ...        &  0 \\
DES\,J233818.71$-$631138.5  &  354.57795  & $ -63.19403 $ &  20.87  &  20.36  &  57568.7  &    7.9  &   \phs$35.2 \pm 1.9$  &  $4.30 \pm 0.83$  &         ...        &  0 \\
DES\,J233821.29$-$631635.7  &  354.58871  & $ -63.27660 $ &  18.49  &  17.70  &  57312.2  &   32.8  &   \phs$19.7 \pm 1.3$  &  $6.73 \pm 0.41$  &         ...        &  0 \\
                            &  354.58871  & $ -63.27660 $ &  18.49  &  17.70  &  57568.7  &   62.3  &   \phs$21.1 \pm 1.0$  &  $6.88 \pm 0.35$  &         ...        &  0 \\
DES\,J233822.94$-$631457.4  &  354.59556  & $ -63.24928 $ &  21.20  &  20.39  &  57312.2  &    4.1  &   \phs$48.3 \pm 5.0$  &         ...       &         ...        &  0 \\
                            &  354.59556  & $ -63.24928 $ &  21.20  &  20.39  &  57568.7  &    8.4  &   \phs$35.4 \pm 1.9$  &  $6.83 \pm 0.56$  &         ...        &  0 \\
DES\,J233824.42$-$631618.0  &  354.60174  & $ -63.27168 $ &  21.26  &  20.75  &  57568.7  &    4.0  &   \phs$28.4 \pm 4.3$  &  $6.09 \pm 1.12$  &         ...        &  0 \\
DES\,J233836.38$-$631544.0  &  354.65157  & $ -63.26221 $ &  17.79  &  17.19  &  57283.3  &   25.6  &      $-26.5 \pm 1.3$  &  $6.08 \pm 0.38$  &         ...        &  0 \\
                            &  354.65157  & $ -63.26221 $ &  17.79  &  17.19  &  57312.2  &   37.0  &      $-26.2 \pm 1.2$  &  $6.15 \pm 0.38$  &         ...        &  0 \\
                            &  354.65157  & $ -63.26221 $ &  17.79  &  17.19  &  57568.7  &   79.9  &      $-26.1 \pm 1.0$  &  $6.74 \pm 0.33$  &         ...        &  0 \\
DES\,J233837.27$-$631441.7  &  354.65530  & $ -63.24491 $ &  20.33  &  20.04  &  57568.7  &    7.1  &  \phs$267.2 \pm 5.3$  &         ...       &         ...        &  0 \\
\enddata
\tablenotetext{a}{Quoted magnitudes represent the weighted-average dereddened PSF magnitude derived from the DES images using SExtractor \citep{drlica15}.}
\tablenotetext{b}{A value of 1 indicates that the star is a member of the relevant satellite, while 0 indicates a non-member.}
\end{deluxetable*}

